Utility-based Resource Allocation and Pricing for Serverless Computing

Serverless computing platforms currently rely on basic pricing schemes that are static and do not reflect customer feedback. This leads to significant inefficiencies from a total utility perspective. As one of the fastest-growing cloud services, serverless computing provides an opportunity to better serve both users and providers through the incorporation of market-based strategies for pricing and resource allocation. With the help of utility functions to model the delay-sensitivity of customers, we propose a novel scheduler to allocate resources for serverless computing. The resulting resource allocation scheme is optimal in the sense that it maximizes the aggregate utility of all users across the system, thus maximizing social welfare. Our approach gives rise to a natural dynamic pricing scheme that is obtained by solving an optimization problem in its dual form. We further develop feedback mechanisms that allow the cloud provider to converge to optimal resource allocation, even when the users' utilities are private and unknown to the service provider. Simulations show that our approach can track market demand and achieve significantly higher social welfare (or, equivalently, cost savings for customers) compared to existing schemes.

==> CPT_non_uniform.tex <==
%!TEX root = main.tex

\section{Lottery-based Resource Allocation}
\label{sec: CPT_model}

In the previous sections, we focused on the importance of taking into account the delay-sensitivity characteristics of the agents while allocating resources in serverless systems.
The purpose of considering delay-sensitivity characteristics was to distinguish between agents who have different QoS (quality-of-service) requirements based on the delay in the execution of their jobs.
We saw how to allocate resources that would prioritize the customers based on their delay-sensitivity requirements and charge them appropriately.
A potential problem of such market-based pricing scheme is that
if the supply of resources exceeds the demand by a lot, then it might drive the prices high and discourage some of the smaller customers from participating in such markets.
Several service providers use lottery-based allocations to decide which agents to serve next.
As a result, all the customers who are willing to pay the minimum price set by the service provider get a shot at receiving services. 
Such lottery-based provisions, however, give rise to uncertainties in the execution of the jobs or their delay times.
Just as we distinguished between different customers with varying delay-sensitivity, another important criteria for the QoS is the uncertainty in execution of jobs, and different agents have different preferences towards these uncertainties.
In practice, it is common to make provisions in the SLAs (service-level-agreements)
to provide compensation to the customers if a certain fraction of their jobs are not executed in time.
Currently, most service providers have a fixed SLA agreement, but such a "one-size fits all" approach is inefficient.
In this section, we show that we can build on our system model to account for such lottery-based allocations.
The concept of utility functions from economics helped us model the delay-sensitivity of the customers.
Now again, economics offers us the notion of probabilistic-sensitivity to model customers' preferences towards uncertainties.


Suppose the uncertain completion time for user $i$ is given by the lottery
\begin{equation}
\label{eq: lottery_form}
     L_i := \{(p_i(1), y_i(1)), \dots, (p_i(K), y_i(K)) \},
\end{equation}
where $y_i(k) \geq 0, k \in [K]$, are the completion times and $p_i(k)$ the corresponding probabilities with which they occur.
We assume the lottery to be exhaustive, i.e. $\sum_{j = 1}^K p_i(k) = 1$.
(Note that we are allowed to have $p_i(k) = 0$ for some values of $k \in [K]$ and $y_i(k) = y_i({k'})$ for some $k, k' \in [K]$.)
A natural approach to account for such uncertainties is to use expected utility instead of the utility corresponding to any single completion time.
Thus the ``happiness'' of user $i$ under expected utility theory (EUT) for lottery $L_i$ will be given by
\[
    \sum_{k = 1}^K p_i(k) U_i(y_i(k) ).
\]


We now consider the multi-tier model with $T$ tiers and $N$ users.
Recall that $\tau_t$ denotes the end time of tier $t$ and $U_{i,t} = U_i(\tau_t)$.
Let $q_{i,t}$ denote the probability that user $i$'s jobs are completed by the end of tier $t$.
Let 
\begin{equation}
\label{eq: cumprob_to_prob}
    p_{i,t} := q_{i,t} - q_{i,(t-1)}
\end{equation}
denote the probability that user $i$'s jobs are completed in tier $t$, i.e., they are completed by the end of tier $t$ but not by the end of tier $(t-1)$.
Suppose we ask that the cloud capacity constraints are satisfied in expectation.
Then this condition can be written as the constraint 
$$\sum_{i = 1}^N p_{i,t} J_i \leq M_t,$$ 
for all $t$.
\vip{Insert some justification here (problem difficult otherwise, cloud provider has reserves) etc.}
The problem of maximizing expected utility with a probabilistic allocation of resources to users is given by
\begin{align}
\text{\bf\underline{SYS-EU}} \nn \\
\max _{p_{i,t} \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{t=1}^{T} p_{i,t} U_{i,t} \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} p_{i,t} \leq 1, \forall i \in[N],\\
 & \sum_{i=1}^{N} p_{i, t} J_{i} \leq M_{t}, \forall t \in[T].
\end{align}
%Here, the system constraints are satisfied on average.


We now observe that SYS-EU is exactly same as SYS-LP with the transformation $x_{i,t} = p_{i,t} J_i$.
Since we know how to solve the problem SYS-LP, we get the solution for SYS-EU.
Further, the sparsity of the solution $\x$ to SYS-LP (see Theorem~\ref{thm:gap_bound}), shows that for most of the users we have a lottery $L_i$ that allocates resources in a specific tier with probability $1$.
Thus, \emph{for most of the users, we assign them deterministic lotteries under EUT}.


Such an allocation scheme would result in discouraging the users who have lower willingness-to-pay as mentioned before.
Consider a user whose willingness-to-pay is $\$1$ to get her job completed in $1$ sec.
Suppose the market price is $\$1.5$ for job completion within $1$ sec.
It is possible that this user is ready to pay $\$0.2$ to get a $10\%$ chance of having her job completed in $1$ sec.
Note that this behavior is different from EUT predictions.
In fact, it has been observed through several empirical studies that individuals often do not behave according to EUT and display varying degrees of sensitivity to probabilities.
Lotteries provide a way to capture such customers in the market.
%In this section, we generalize our system model to consider probabilit
The correct model to consider to analyse this phenomenon is cumulative prospect theory (CPT) \cite{tversky1992advances}, a generalization of expected utility, and one of the leading decision theory models.
It allows us to capture the probabilistic-sensitivity of the customers.



We now describe the CPT model that we use to measure the ``happiness'' derived by each player from her lottery (for more details see~\cite{wakker2010prospect}). 
Suppose an agent faces a lottery $L_i$ as shown in \eqref{eq: lottery_form}.
%$$L = \{(p(1), y(1)), \dots, (p(k), y(k)) \},$$
%where $y_j \in \bbR^+$ are the end times and $p_j$ the corresponding probabilities with which they occur.
%We assume the lottery to be exhaustive, i.e. $\sum_{j = 1}^k p^j = 1$.
%
%It is a generalization of the expected utility theory model (EUT) \citep{von1945theory} of choice under risk, 
%and a special case of cumulative prospect theory (CPT) \citep{tversky1992advances}.
Each player $i$ is associated with a utility function
%\footnote{
%The value function in RDU is generally defined on $\bbR$. However, since we will be dealing only with nonnegative throughputs, we restrict it to $\bbR_+$.
%}
$u_i : \bbR_+ \to \bbR_+$ 
as before, 
and a probability weighting function $w_i : [0,1] \to [0,1]$ that is continuous, 
%\footnote{
%The continuity assumption for the probability weighting function can be relaxed. Discontinuities at $0$ and $1$ are empirically interesting 
%(for more on the phenomenon of ignorance at end points see 
%\citep{kahneman1979prospect}. 
%}
strictly increasing and satisfies $w_i(0) = 0$ and $w_i(1) = 1$. 



For the prospect $L_i$, let $\pi_i : [K] \to [K]$ be a permutation such that
\begin{equation}
	\label{eq: pi_order_1}
	U_i(\bar y_i(1) ) \geq U_i(\bar y_i(2)) \geq  \dots \geq U_i(\bar y_i(K)),
\end{equation}
and
\begin{equation}
	\label{eq: pi_order_2}
	\bar y_i(k) := y_i({\pi_i(K)}) \mbox{ for all } k \in [K].
\end{equation}
This is equivalent to the ordering 
\[
    \bar y_i(1) \leq \bar y_i(2) \leq  \dots \leq \bar y_i(k),
\]
since the utility function $U_i(\cdot)$ is assumed to be decreasing.
The prospect $L_i$ can equivalently be written as
\[
	L_i = \{(\bar p_i(1), \bar y_i(1)); \dots ; (\bar p_i(k), \bar y_i(k))\},
\]
where $\bar p_i(k) := p_i({\pi_i(k)})$ for all $k \in [K]$.
The \emph{CPT value} of prospect $L_i$ for the agent is evaluated using the utility function $U_i(\cdot)$ and the probability weighting function $w_i(\cdot)$ as follows:
\begin{equation}
\label{eq: RDU_formula}
	V_i(L) := \sum_{k = 1}^{K} d_i(p_i,\pi_i, k)U_i(\bar y_i(k)),
\end{equation}
where $d_i(p_i,\pi_i, k)$ are the \emph{decision weights} given by $d_i(1)(p_i,\pi_i) := w_i(\bar p(1))$ and
\begin{align*}
	d_i(p_i,\pi_i, k) := w_i(\bar p_i(1) + \dots + \bar p_i(k)) - w_i(\bar p_i(1) + \dots + \bar p_i({k - 1})),
\end{align*}
for $1 < k \leq K$.
Although the expression on the right in equation \eqref{eq: RDU_formula} depends on the permutation $\pi_i$, one can check that the formula evaluates to the same value $V_i(L_i)$ as long as $\pi_i$ satisfies \eqref{eq: pi_order_1} and \eqref{eq: pi_order_2}. 
The CPT value of prospect $L_i$, can equivalently be written as
\[
	V_i(L_i) = \sum_{k = 1}^{K} w_i\big(\sum_{s = 1}^{k} \bar p_i^s\big ) \l[ U_i(\bar y_i(k)) - U_i(\bar y_i({k + 1})) \r],
\]
where $\bar y_i({K+1}) := 0$.
Thus the worst end time $\bar y_i({K})$ is weighted by $w_i(1) = 1$, and every increment in the value of the allocations, $U_i(\bar y_i(k)) - U_i(\bar y_i({k + 1})), \forall k \in [K -1]$, is weighted by the probability weighting function of the probability of receiving an allocation at least equal to $\bar y_i(k)$.

Some example of weighing functions are provided in Figure \ref{fig:cpt_weighing}.
% \sph{@Vipul It would be nice to have plots for different values of $\gamma_i$ in the same figure.}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.31\textwidth}
        \centering
        \includegraphics[scale=0.5]{figs_cpt/PL_curve.pdf}
        \caption{ A piecewise linear weighing function}
        \label{fig:PL_cpt}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.31\textwidth}
        \centering
        \includegraphics[scale=0.5]{figs_cpt/log_curve.pdf}
        \caption{ $w_{i}(p)=\exp \left\{-(-\ln p)^{\gamma_{i}}\right\}$}
    \end{subfigure}
     ~
    \begin{subfigure}[t]{0.31\textwidth}
        \centering
        \includegraphics[scale=0.5]{figs_cpt/2_param_curve.pdf}
        \caption{  $w_{i}\left(p_{i}\right)=\frac{\delta p_{i}^{ \gamma_{i}}}{\delta p^{\gamma_{i}}+(1-p)^{\gamma_{i}}}, \delta=0.7$}
        \label{fig:2param_cpt}
    \end{subfigure}
    \caption{Different parametric families to model CPT weightings.}
\label{fig:cpt_weighing}
\end{figure*} 

%Now, let us define $q_{i t}=\sum_{\tau=1}^{t} p_{i \tau}$ as the cumulative probabilities and let $w_i(\cdot)$ as the weighing function (see Fig. \ref{fig:cpt_weighing} for examples). 
Let us now consider the multi-tier based model.
Recall that the difference in the utilities of job completion in tiers $t$ and $t+1$ is given by $u_{i,t} = U_{i,t} - U_{i,{t+1}}$.
Then, the CPT based system problem is given by
\begin{align}
\text{\bf\underline{SYS-CPT}} \nn \\
\max _{p_{i,t}, q_{i,t} \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{t=1}^{T} w_{i}\left(q_{i, t}\right) u_{i, t} \label{eq: sys_cpt_0}\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} p_{i, t} \leq 1, \forall i \in[N],\label{eq: sys_cpt_1}\\
 & \sum_{i=1}^{N} p_{i, t} J_{i} \leq M_{t}, \forall t \in[T],\label{eq: sys_cpt_2}\\
 & q_{i, t}=\sum_{s=1}^{t} p_{i, s}, ~\forall~ i \in[N], t \in[T].
\end{align}
%where $u_{i t}=U_{i}^t-U_{i}^{t+1}$.



\sph{Include a discussion on the non-convexity of the problem SYS-CPT in general. @Vipul Can we include some results from simulation to show that there are several local optima and in general it is hard to find the optimum?
Create a section in Appendix where we show that this problem is hard to solve in general. This will clarify why we are looking at the dicretized version next.}

%\vip{@soham Why talk about uniform quantization at all? Should we just redo the entire thing with non-uniform quantization?}




We now use the discretization trick introduced in \cite{phade2019optimal} to solve SYS-CPT approximately.
Besides there are behavioral reasons to adopt such a discretization. 
We will explain them shortly.
Let us first describe the discretization trick.
Fix an integer $K > 0$.
We restrict our attention to lotteries where each agent is shown probabilities from a finite set.
In particular, we will assume that the cumulative probabilities shown to the agents satisfy
\begin{equation}
    q_{i,t} \in \l\{\frac{k}{K}: 0 \leq k \leq K \r\} =: \Delta.
\end{equation}
Notice that this implies
\begin{equation}
    p_{i,t} \in \l\{\frac{k}{K}: 0 \leq k \leq K \r\} = \Delta.
\end{equation}
%Thus, we  only the probabilities belonging to the discretized mesh $\Delta$.
As $K \to \infty$, we get better approximations to any probability distribution.
However, there is a practical motivation to keep $K$ limited.
From a behavioral perspective, people often do not comprehend small differences in probability.
For this reason, it is useful to restrict $K$ (for example $K \leq 100$).


Although we restrict ourselves to showing the agents probabilities belonging to the discretized mesh $\Delta$, it does not stop us from using implementations with general probabilities as long as we are providing the agents at least what we are promising them.
Let us make this argument concrete.
Suppose we show each player $i$ a lottery $L_i$ with cumulative probabilities 
\[
    q_{i,\bullet} := (q_{i,t})_{t \in [T]},
\] 
and corresponding probabilities 
\[
    p_{i,\bullet} := (p_{i,t})_{t \in [T]},
\] 
satisfying \eqref{eq: cumprob_to_prob}.
Suppose we use an implementation defined by probabilities $\hat \p := (\hat p_{i,t})_{i, t}$, where $\hat p_{i,t}$ denotes the probability with which player $i$ is allocated her resources $J_i$ in tier $t$.
Thus the true lottery $\hat L_i$ for player $i$ is given by $\hat p_{i,\bullet} = (\hat p_{i,t})_{t}$ and the corresponding cumulative probabilities $\hat q_{i, \bullet} := (\hat q_{i,t})_{t}$, where $\hat q_{i,t} = \sum_{\tau = 1}^t \hat p_{i\tau}$.
We use the notion of first order stochastic dominance to determine when one lottery is better than the other.
Lottery $\hat L_i$ first order stochastically dominates lottery $L_i$ if
\[
    \hat q_{i,t} \geq q_{i,t}, \forall t \in [T].
\]
Note that, if lottery $\hat L_i$ first order stochastically dominates lottery $L_i$, then lottery $\hat L_i$ is formed by shifting probability mass from some outcomes to outcomes that are strictly preferred to them.
This is a very strong condition of dominance and it is widely held that any satisfactory theory of preferences should satisfy it \cite{starmer2000developments}.
In particular, the CPT preferences and EUT preferences satisfy this condition.


Thus, we ask that $\hat \p$ is implementable, i.e. it satisfies the capacity constraints \eqref{eq: sys_cpt_1} and \eqref{eq: sys_cpt_2}.
For each player $i$, lottery $\hat p_{i, \bullet}$ first order stochastically dominates lottery $p_i$.
The probabilities $p_{i,t}$ belong to the mesh $\Delta$.
Let us call this discretized version of SYS-CPT as SYS-CPT-K that is given by
%\vip{SYS-CPT-K is not mentioned anywhere.}
\begin{align}
\text{\bf\underline{SYS-CPT-K}} \nn \\
\max _{\hat p_{i,t} \geq 0, q_{i,t}\in \Delta } ~~~~~& \sum_{i=1}^{N} \sum_{t=1}^{T} w_{i}\left(q_{i, t}\right) u_{i, t} \label{eq: sys_cpt_k_0}\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} \hat p_{i t} \leq 1, \forall i \in[N]\label{eq: sys_cpt_k_1}\\
 & \sum_{i=1}^{N} \hat p_{i, t} J_{i} \leq M_{t}, \forall t \in[T],\label{eq: sys_cpt_k_2}\\
 &\sum_{s=1}^{t} \hat p_{i, s} \geq  q_{i t}, ~\forall~ i \in[N], t \in[T].
\end{align}





{\bf A richer problem formulation:}
We now give a richer problem formulation that would help us solve the above discretized version of SYS-CPT.
Suppose the cloud provider achieves a lottery implementation through a scheme as follows: 
The scheduler implements with equal probability one of the $K$ allocation schemes $x_{\bullet, \bullet}(k) := (x_{i,t}(k)), i \in [N], t \in [T]$, for $k \in [K]$.
Let $[K]$ denote the set of \emph{alternatives}.
For alternative $k$, the job end time for user $i$ is given by
\vip{Some typo below?}
\begin{equation}
\label{eq: cpt_end_time_def}
    T_i(k) := \min \{t \in [T] : \sum_{s = 1}^t x_{i,s}(k) \geq J_i \},
\end{equation}
Thus the probability that user $i$'s jobs are completed by the end of tier $t$ is given by
\begin{equation}
    \label{eq: cpt_endT_to_cum_prob}
    q_{i,t} = \frac{|\{k: T_i(k) \leq t \}|}{K},
\end{equation}
and the lottery faced by user $i$ is given by
\begin{align*}
    L_i = \{(p_{i,1}, \tau_1); \dots; (p_{i,T}, \tau_T)\},
\end{align*}
where 
\begin{equation}
%\label{eq: cumprob_prob}
   p_{i,t} = q_{i,t} - q_{i,(t-1)}. 
\end{equation}
The CPT value of this lottery is
\begin{align}
\label{eq: CPT_val_1}
    V_i(L_i) = \sum_{t = 1}^T w_i(q_{i,t}) u_i^t.
\end{align}
This lottery can equivalent be written as
\begin{align*}
    L_i = \{({1}/{K}, \tau_{T_i(1)});\dots;({1}/{K}, \tau_{T_i(k)})\}.
\end{align*} 
Note that in this formulation the end times can appear repeatedly, but the total probability of any particular end time is same in both the formulations.
It is easy to verify that CPT value formula is invariant under such equivalent representations.
Also note that the end times in the second formulation are not ordered.
Let $\pi_i: [K] \to [K]$ be a permutation such that
\[
    {\bar T_i(1)} \leq {\bar T_i(2)} \leq  \dots \leq {\bar T_i(k)},
\]
where $\bar T_i(k) = T_i({\pi_i(k)})$.
Then the CPT value of user $i$ for lottery $L_i$ is given by
\begin{align}
\label{eq: CPT_value_2}
     V_i(L_i) = \sum_{k = 1}^K h_i(k) U_i^{\bar T_i(k)}.
\end{align}
where $h_i(k) := w_i(k/K) - w_i((k-1)/K)$ for $k \in [K]$.
Note that the two formulas for the CPT value in \eqref{eq: CPT_val_1} and \eqref{eq: CPT_value_2} are equivalent.
Also note that if $w_i(\cdot)$ is an identity function (as in the EUT setting), then $h_i(k) = 1/K$, and the corresponding CPT value is simply the average of the utility from all alternatives. 
%
% Note that when $w_i(0) = 0 ~\forall ~i\in [N]$, the objective in EU-CPT can be equivalently written as
% $$\max _{q_{i t} \geq 0} \sum_{i=1}^{N} \sum_{t=1}^{T} \left(w_{i}q_{it} - w_{i}q_{i(t-1)}\right) U_{i}^t.$$
%
% Let us consider an alternate formulation of EU-CPT, where the cloud provider has $K$ alternatives, with the $k$-th alternative corresponding to a resource allocation matrix $\x(k)\in \R^{N\times T}, k\in [K],$ according to which the $N$ users are allocated resources across $T$ tiers. Now, instead of optimizing over cumulative probabilities ($q_{it}$'s), let us optimize over the $K$ alternatives, and hope that the resulting problem will be convex.
%
% Also, let us define the incremental CPT weightings as
% $$ h_i(k) = w_i\l(\frac{k}{K}\r) - w_i\l(\frac{k-1}{K}\r) ~\forall ~k \in [K], i\in [N].$$
%


We now use the relaxation trick as in the previous section.
We approximate the utility for user $i$ corresponding to alternative $k$ as follows:
\begin{align}
\label{eq: cpt_approx}
    U_i^{T_i(k)} \approx \sum_{t = 1}^T \frac{x_{it}^k U_i^t}{J_i}.
\end{align}
Note that when $(x_{it}(k), t \in [T])$ is $1$-sparse with that non-zero entry equal to $J_i$, the above approximation is exact.
With this relaxation our objective can be written as
\[
    \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) \bP_i(x_{i, \bullet}({\pi_i(k)}) ),
\]
where $\bP(x_{i, \bullet}(k) ) = \sum_{t=1}^T x_{it}(k) P_{it} = \sum_{t=1}^T x_{it}(k) U_i^t/J_i$ and the permutation $\pi_i(k)$ is such that
\begin{equation}
\label{eq: pi_bar_P_ineq_x}
    \bP_i(x_{i, \bullet}({\pi_i(1)}) ) \geq \bP_i(x_{i, \bullet}({\pi_i(2)}) ) \geq \cdots \geq \bP_i(x_{i, \bullet}({\pi_i(K)})),
\end{equation}
for all $i$.



Corresponding to allocations $x_{\bullet, \bullet}(k), \forall k \in [K]$ and permutations $\pi_i, \forall i \in [N]$, let $z_{it}(k) := x_{it}({\pi_i(k)})$ be a $|T|$-dimensional column vector, for $i \in [N], k \in [K]$.
With this notation, the objective function can be written as
\begin{equation}
    \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) \bP_i(z_{i, \bullet}(k)),
\end{equation}
and the inequalities~\eqref{eq: pi_bar_P_ineq_x} take the form
\begin{equation}
    \bP_i(z_{i, \bullet}(1)) \geq \bP_i(z_{i, \bullet}(2)) \geq \cdots \geq \bP_i(z_{i, \bullet}(k)),
\end{equation}
for all $i$.

Strictly speaking, such a scheme in our richer problem formulation is feasible iff each of the alternatives is feasible, i.e. 
\begin{equation}
\label{eq: feasibility_hard_constraint}
    \sum_{i = 1}^N x_{it}(k) \leq M_t
\end{equation}
for all $t, k$. However, we will use this richer formulation only as an intermediate step to solve the discretized SYS-CPT problem (namely, SYS-CPT-K) where we are interested in the implementations that are feasible in expectation. 
Hence we will, instead, consider the constraint 
\begin{equation}
    \frac{1}{K} \sum_{k = 1}^K \sum_{i = 1}^N x_{it}(k)  \leq M_t, \forall t \in [T].
\end{equation}

This motivates the following relaxed system problem:
\begin{align}
\text{\bf\underline{SYS-CPT-K-R}} \nn \\
\max _{\z(k) \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) \bP_i(z_{i, \bullet}({k})) \label{eq: sys_cpt_lp_r_0}\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}(k) \leq J_i, ~\forall~ i \in[N], k \in [K], \label{eq: sys_cpt_lp_r_1}\\
 &\frac{1}{K} \sum_{k=1}^K\sum_{i=1}^{N} z_{it}(k) \leq M_{t}, ~\forall ~t \in[T],\label{eq: sys_cpt_lp_r_2}\\
 &\bP_i(z_{i, \bullet}({k})) \geq \bP_i(z_{i, \bullet}({k+1})), ~\forall~i \in [N], ~\forall ~1 \leq k \leq K-1. \label{eq: sys_cpt_lp_r_3}
\end{align}


Notice that the problem SYS-CPT-K-R is an LP problem.
As compared to the previous problems SYS-CPT and SYS-CPT-K, the number of variables in SYS-CPT-K-R has become $K$-fold.
Although this might seem like a problem from a computational point of view, later we will derive some qualitative features about the optimal solution which will let us significantly reduce the dimensions of our variables.
But more on this later.
Let us first observe how the solution to SYS-CPT-K-R compares to the solution to SYS-CPT-K.

% Besides, the value of the problem SYS-CPT-K-R is equal to the value of the problem SYS-CPT-K-2.
% (Further details relating the primal and dual values the problems SYS-CPT-K-2, SYS-CPT-3 and SYS-CPT-R can be found in \cite{phade2019optimal}).
%Let us now compare the constraint \eqref{eq: sys_cpt_1} with \eqref{eq: sys_cpt_lp_r_1} and the contraint \eqref{eq: sys_cpt_2} with \eqref{eq: sys_cpt_lp_r_2}.
Suppose $\hat p_{it}^*, q_{it}^* \in \Delta$ is an solution to the SYS-CPT-K problem.
Then, let us construct a corresponding lottery allocation $\z^*$ as follows: let 
\begin{equation}
\label{eq: q_to_z}
     z_{it}^*(k) = \begin{cases}
        J_i, &\text{ if } q_{i(t-1)} < k/K \leq q_{it},\\
        0, &\text{ otherwise,}
    \end{cases}
\end{equation}
for all $i, t, k$.
(Recall that $q_{it} \in \Delta$.)
One can verify that $\z^*$ is a feasible solution to SYS-CPT-K-R, and the objectives \eqref{eq: sys_cpt_lp_r_0} and \eqref{eq: sys_cpt_0} match exactly.
This is because the allocations $z_{i, \bullet}^*(k)$ are $1$-sparse with the non-zero entry equal to $J_i$, and hence
the approximation in \eqref{eq: cpt_approx} is exact.
%In particular, suppose $\hat p_{it}^*, q_{it}^* \in \Delta$ is an optimal solution to the SYS-CPT-K problem, then 
Further, the optimal value of SYS-CPT-K matches
\begin{equation}
    V^* := \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) \bP_i({z_{i, \bullet}^*(k)}).
\end{equation}
%where $\z^*$ is defined from $q^*$ similar to \eqref{eq: q_to_z}.

On the other hand, let $\z^R$ be the optimal solution of SYS-CPT-K-R.
Let $V^R$ denote the optimal value of the objective function of SYS-CPT-K-R, i.e.
\begin{equation}
    V^R := \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) \bP_i({z_{i, \bullet}^R({k})}).
\end{equation}
 We now define the end times $\tilde T_i(k)$ for each player $i$ for her $k$th best alternative by
\begin{equation}
\label{eq: cpt_end_time_def_k_best}
    \tilde T_i(k) := \min \{t \in [T] : \sum_{\tau = 1}^t {z_{i,\tau}^R(k)} \geq J_i \},
\end{equation}
similarly to \eqref{eq: cpt_end_time_def}.
Now consider $\tilde q_{it}$ given by
\begin{equation}
    \label{eq: cpt_endT_to_cum_prob_k_best}
    \tilde q_{it} := \frac{|\{k: \tilde T_i(k) \leq t \}|}{K},
\end{equation}
similar to \eqref{eq: cpt_endT_to_cum_prob}.
Finally, let 
\begin{equation}
\label{eq: tilde_q_to_tilde_z}
     \tilde z_{it}(k) = \begin{cases}
        J_i, &\text{ if } \tilde q_{i(t-1)} < k/K \leq \tilde q_{it},\\
        0, &\text{ otherwise,}
    \end{cases}
\end{equation}
similarly to \eqref{eq: q_to_z}.
Let the value of the objective function in SYS-CPT-K-R corresponding to $\tilde z$ be
\begin{equation}
    \tilde V := \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) \bP_i(\tilde z_{i, \bullet}({k})). 
\end{equation}
Now note that in the allocation $\tilde z$, the players get resources only in their completion tier.
Thus, they do not get any partial utility in our approximation \eqref{eq: cpt_approx}.
Hence, we have that $\tilde V \leq V^R$.
Further, $\tilde V$ is equal to the value of the objective function in SYS-CPT-K corresponding to $\tilde \q$, i.e.
\begin{equation}
    \tilde V = \sum_{i=1}^{N} \sum_{t=1}^{T} w_{i}\left(\tilde q_{i t}\right) u_{i t}.
\end{equation}
We have this because the allocations $\tilde z_{i, \bullet}(k)$ are $1$-sparse with the non-zero entry equal to $J_i$.
Now, if we let
\begin{equation}
     \hat p_{it}^R := \frac{1}{K} \sum_{k = 1}^K {z_{it}^R(k)},
\end{equation}
then $p_{it}^R, \tilde q_{it}$ is a feasible solution to SYS-CPT-K with value $\tilde V$.
Thus $\tilde V \leq V^*$, since $V^*$ is an optimal solution to SYS-CPT-K.

Together, we get that
\begin{equation}
\label{eq: cpt_value_ineq}
    \tilde V \leq V^* \leq V^R.
\end{equation}
In Theorem~\ref{thm:cpt_gap_bound}, we bound the gap between $V^R$ and $V^*$ and thus get a bound on the gap between the optimal solution to SYS-CPT-K and the solution arising from our relaxation.



   


% On the other hand, if we take
% \[
%     p_{it} = \frac{1}{K} \sum_{k = 1}^K z_{it}^k,
% \]
% then, we observe that a feasible solution $z_{it}^k$ to SYS-CPT-K-R gives rise to a feasible solution to SYS-CPT.
% \sph{@Vipul We should simulate and compare these two solutions.}


% In Appendix~\ref{sec: hard_const_relax}, we set up the richer problem formulation and require that the \emph{hard feasibility constraints} hold as in ~\eqref{eq: feasibility_hard_constraint}. However, this problem is NP-hard because it requires an optimal permutation $\pi_i(k)$ to allocate the lotteries.
% Treating the permuations as matrices and relaxing them to be doubly stochastic matrices we get SYS-CPT-R.
% Besides, as proved in \cite{phade2019optimal}, the dual value of the richer problem formulation with hard costraints is equal to the value of the problem SYS-CPT-K-R.


We will now prove certain qualitative features of the optimal solution to SYS-CPT-K-R that we had promised earlier.
These will shed light on the optimal lottery allocations and help us bound the gap between the optimal solutions to SYS-CPT-K and SYS-CPT-K-R.
Besides, it will significantly reduce the dimension of our problem SYS-CPT-K-R making it practical for actual deployment.
This is what allows us to run our simulations.


To describe these qualitative features let us define few parameters of interest related to the probability weighting functions $w_i, \forall i$.
First we impose some additional conditions on the probability weighting functions that are typically based on empirical evidence and psychological arguments \cite{kahneman2013prospect}.
We assume that the probability weighting function $w_i(p_i)$ is concave for small values of the probability $p_i$, say for $p_i \in [0,\tilde p_i]$, and convex for the rest.
Typically the point of inflection is around $1/3$.
Let $w_i^*: [0,1] \to [0,1]$ be the minimum concave function that dominates $w_i$, i.e. $w_i^*(p_i) \geq w_i(p_i)$ for all $p_i \in [0,1]$. Let $p_i^* \in [0,1]$ be the smallest probability such that $w_i^*(p_i)$ is linear over the interval $[p_i^*, 1]$.
It is proved in \cite{phade2019optimal} that $p_i^* \leq \tilde p_i$, and 
\[
    w_i^*(p_i) = w_i(p_i)  \text{ for } p_i \in [0, p_i^*].
\]
Further, if $p_i^* < 1$, then for any $p_i(1) \in [p_i^*, 1)$, we have
\[
    w_i(p_i) \leq w_i(p_i(1)) + (p_i - p_i(1))\frac{1 - w_i(p_i(1))}{1 - p_i(1)},
\]
for all $p_i \in [p_i(1),1]$.

We will now show that the optimal solution $\z$ to SYS-CPT-K-R satisfies
\begin{equation}
\label{eq: low_slab_same}
    \bar P_i(z_i({k^*})) = \bar P_i(z_i({k^* + 1})) = \dots = \bar P_i(z_i({K})),
\end{equation}
where $k^* := \min\{k \in [K]: (k-1)/K \geq p_i^* \}$, provided $p_i^* \leq (K-1)/K$.
Further, if for the optimal solution $\z$, we have $\bar P_{i}(\z_i(k)) = \bar P_{i}(z_{i, \bullet}^{k+1})$, then consider the allocation $\tilde \z$ such that 
$$\tilde z_{i, \bullet}(k) = \tilde z_{i, \bullet}({k+1}) = \frac{z_{i, \bullet}(k) +  z_{i, \bullet}({k+1})}{2},$$
and $\tilde \z$ is same as $\z$ everywhere else.
Note that $\tilde \z$ is also an optimal solution to SYS-CPT-K-R.
Thus, we have

\begin{proposition}
\label{prop: typical_lottery}
    There exists an optimal solution $\z$ to SYS-CPT-K-R such that \eqref{eq: low_slab_same} holds for all the players $i$, and whenever $\bar P_{i}(z_{i, \bullet}(k)) = \bar P_{i}(z_{i, \bullet}(k+1))$, we have $z_{i, \bullet}(k) = z_{i, \bullet}({k+1})$.
\end{proposition}
We prove this proposition in the Appendix~\ref{prop: typical_lottery}.


% As a consequence of this result, we will consider a discretization in which
% \[
%     p_{it} \in \{0,\epsilon_1, \epsilon_2, \dots, \epsilon_L\} \text{ for all } i\in [N], t\in [T],
% \]
% where $L$ denotes the different levels of quantization we want. For example, we can have $L=2$ with $p_{it} \in \{0,0.05, 0.4\}$. For such a discretization, we have 
% $$q_{it} \in \{0, \delta_1, \delta_2, \cdots, \delta_K\}, \text{ for all } i\in [N], t\in [T], $$
% where $K$ is the number of points considered for discretization. For the previous example with $L=2$ and $p_{it} \in \{0.05, 0.4\}$,
% one possible instantiation of this set is $q_{it} \in \{0.05, 0.1, 0.15, 0.2, 0.6, 1\}$. In general, $q_{it} = \sum_{\tau=1}^t p_{i\tau} = \sum_{\tau=1}^t \epsilon_{i\tau}$, where $\epsilon_{i\tau}\in \{0,\epsilon_1, \dots, \epsilon_L\}$. \vip{Better way to explain?}

In the following, we will establish the sparsity of the optimal solution $z$ to SYS-CPT-K-R, and use this to bound the gap between the optimal solutions of SYS-CPT-K and SYS-CPT-K-R.
But before that, let us take a closer look at the problem SYS-CPT-K-R.







% With this interpretation in terms of $[K]$ alternatives, we get the following problem:
% \begin{align}
% \text{\bf\underline{SYS-CPT-K}} \nn \\
% \max_{\substack{
% \x(k) \geq 0,\forall k,\\
% \pi_i,\forall i,\\
% T_i(k), \tilde T_i(k), \forall i,k 
% }} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) U_i^{\tilde T_i(k)} \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} x_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K],\\
%  & \sum_{i=1}^{N} x_{it}^k \leq M_{t}, ~\forall ~t \in[T], k \in [K],\\
%  & T_i(k) := \min \{t \in [T] : \sum_{s = 1}^t x_{is}^k \geq J_i \}, ~\forall~i \in [N], k \in [K],\\
%  & \tilde T_i(k) = T_i^{\pi_i(k)},~\forall~i \in [N], k \in [K],\\
%  & {\tilde T_i(1)} \leq {\tilde T_i(2)} \leq  \dots \leq {\tilde T_i(k)}, ~\forall i \in [N].
% \end{align}

% We now use the relaxation trick as in the previous section.
% We approximate the utility for user $i$ corresponding to alternative $k$ as follows:
% \begin{align}
% \label{eq: cpt_approx}
%     U_i^{T_i(k)} \approx \sum_{t = 1}^T \frac{x_{it}^k U_i^t}{J_i}.
% \end{align}
% Note that when $(x_{it}^k, t \in [T])$ is $1$-sparse with that non-zero entry equal to $J_i$, the above approximation is exact.
% With this relaxation our problem can be written as
% \begin{align}
% \text{\bf\underline{SYS-CPT-K-1}} \nn \\
% \max _{\x(k) \geq 0, \pi_i} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) \bP_i(\x_{i}^{\pi_i(k)}) \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} x_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K],\\
%  & \sum_{i=1}^{N} x_{it}^k \leq M_{t}, ~\forall ~t \in[T], k \in [K],
% \end{align}
% where $\bP(\x_{i}^k) = \sum_{t=1}^T x_{it}^k P_{it} = \sum_{t=1}^T x_{it}^k U_i^t/J_i$ and the permutation $\pi_i(k)$ is such that
% $$ \bP_i(\x_i^{\pi_i(1)}) \geq \bP_i(\x_i^{\pi_i(2)}) \geq \cdots \geq \bP_i(\x_i^{\pi_i(K)}).$$
% Note that the non-convex function $w_i(\cdot)$ is represented in the relaxed problem as constants $h_i(k)$ due to discretization. However, the relaxed problem is still NP-hard since it requires an optimal permutation $\pi_i(k)$ to allocate the lotteries (we will discuss more on how to allocate lotteries with this formulation later). 

% We now further relax the above problem by using the trick from \cite{phade2019optimal}.
% This involves re-writing the problem by representing the permutations as a permutation matrix and relaxing them to doubly stochastic matrices.
% We now give the details of this transformation.
% %This gives rise to the following problem (see~\cite{phade2019optimal} for details of this transformation):
% Corresponding to allocations $\x(k), \forall k \in [K]$ and permutations $\pi_i, \forall i \in [N]$, let $z_{it}^k := \x_{it}^{\pi_i(k)}$ be a $|T|$-dimensional column vector, for $i \in [N], k \in [K]$, and let $S_i$ be the $K \times K$ matrix given by $S_i(s,t) = 1$ if $\pi_i(t) = s$ and $S_i(s,t) = 0$ otherwise, for $s,t \in [K], i \in [N]$.
% Note that $S_i$ is the permutation matrix corresponding to the permutation $\pi_i^{-1}$~(i.e. inverse of the permutation $\pi_i$).
% Note that $S_i$ is also a doubly stochastic matrix.
% Let $\Omega_K$ denote the set of all $K \times K$ doubly stochastic matrices, and
% let $\Omega_K^*$ denote the set of all $K \times K$ permutation matrices.
% Also note that the allocations $\x(k), \forall k \in [K]$ and the permutations $\pi_i, \forall \in [N]$ are uniquely defined by $\z := (z_{it}^k, i \in [N], t \in [T], k \in [K])$, and $S_i, i \in [N]$.
% Let $\z_i(k) := (z_{it}^k, t \in [T])$ and $\z_{it} := (z_{it}^k, k \in [K])$ denote column vectors.
% Let $\1$ denote a column vector of dimension $K$.
% The problem SYS-CPT-K-1 can equivalently be written as follows:
% \begin{align}
% \text{\bf\underline{SYS-CPT-K-2}} \nn \\
% \max_{\z \geq 0, S_i \in \Omega_K^*} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) \bP_i(\z_i(k)) \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K],\\
%  & \sum_{i=1}^{N} S_i \z_{it} \leq M_{t} \1, ~\forall ~t \in[T],\\
%  &\bP_i(\z_i(1)) \geq \bP_i(\z_i(2)) \geq \cdots \geq \bP_i(\z_i(k)).
% \end{align}

% We now relax the constraint $S_i \in \Omega_K^*$ to be $S_i \in \Omega_K$.
% This gives us the following problem:
% \begin{align}
% \text{\bf\underline{SYS-CPT-K-3}} \nn \\
% \max_{\z \geq 0, S_i \in \Omega_K} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) \bP_i(\z_i(k)) \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~ i \in[N],\\
%  & \sum_{i=1}^{N} S_i \z_{it} \leq M_{t} \1, ~\forall ~t \in[T],\label{eq: sys_cpt_k_3}\\
%  &\bP_i(\z_i(1)) \geq \bP_i(\z_i(2)) \geq \cdots \geq \bP_i(\z_i(k)).
% \end{align}

% Notice that the constraint $\sum_{i=1}^{N} S_i \z_{it} \leq M_{t}$ implies that 
% \[
%     \frac{1}{K} \sum_{k=1}^K \sum_{i=1}^{N} z_{it}^k = \frac{1}{K} \sum_{i=1}^{N} \1^T S_i z_{it} \leq \1^T M_t \1 \leq M_t.
% \]
% If we replace constraint \eqref{eq: sys_cpt_k_3} by the above condition we get
% \begin{align}
% \text{\bf\underline{SYS-CPT-K-R}} \nn \\
% \max _{\z(k) \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i(k) \bP_i(\z_{i}^{k}) \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K], \label{eq: sys_cpt_lp_r_1}\\
%  &\frac{1}{K} \sum_{k=1}^K\sum_{i=1}^{N} z_{it}^k \leq M_{t}, ~\forall ~t \in[T],\label{eq: sys_cpt_lp_r_2}\\
%  &\bP_i(\z_i^{k}) \geq \bP_i(\z_i^{k+1}), ~\forall~i \in [N], ~\forall ~1 \leq k \leq K-1. \label{eq: sys_cpt_lp_r_3}
% \end{align}






%Here, we relaxed the constraints such that the system and user job constraints are satisfied on average (as in the EU problem). Now, the idea is to show that the overall CPT utility of the system through the three problems is almost the same, that is, EU-CPT-R2 $\approx$ EU-CPT-R $\approx$ EU-CPT

%{\bf Sparsity of optimal lottery allocation:}
Let $\lambda_i(k), \mu^t, \alpha_i(k)$ denote the dual variables corresponding to the constraints \eqref{eq: sys_cpt_lp_r_1}, \eqref{eq: sys_cpt_lp_r_2}, and \eqref{eq: sys_cpt_lp_r_3}.
The complementary slackness conditions for the SYS-CPT-K-R problem are:
\begin{align}
\label{cpt_sys_kkt1} 
h_{i}(k) P_{it} - \lambda_i(k) - \frac{\mu_t}{k} + P_{it} (\alpha_i(k) - \alpha_i^{k-1})
&\begin{cases}
= 0, & \text{ if } z_{it}(k) > 0,\\
\geq 0, & \text{ if } z_{it}(k) = 0,
\end{cases}
\quad \quad \forall i, t,\\
\label{cpt_sys_kkt2} 
\sum_{t = 1}^T z_{it}(k) 
&\begin{cases}
= J_i, & \text{ if } \lambda_i(k) > 0,\\
\leq J_i, & \text{ if } \lambda_i(k) = 0,
\end{cases}
\quad \quad ~\forall i,k,\\
\label{cpt_sys_kkt3}
\frac{1}{K}\sum_{i=1}^N \sum_{k=1}^{K} z_{it}(k) 
&\begin{cases}
= M_t, & \text{ if } \mu_t > 0,\\
\leq M_t, & \text{ if } \mu_t = 0,
\end{cases}
\quad \quad ~~~\forall t,\\
\label{cpt_sys_kkt4}
\sum_{t=1}^T P_{it} z_{it}(k) -  \sum_{t=1}^T P_{it} z_{it}({k+1}) 
&\begin{cases}
= 0, & \text{ if } \alpha_i(k) > 0,\\
\geq 0, & \text{ if } \alpha_i(k) = 0,
\end{cases}
\quad \quad ~~~\forall i, k.
\end{align}
Now observe that $\alpha_i(0) = \alpha_i(k) = 0$ for all $i$.
Consider the set $\cal{S}_i$ comprising of elements $(k_1, k_2; i)$ such that $0 < k_1 \leq k_2 < K$, $\alpha_i({k_1 - 1}) = \alpha_i({k_2}) = 0$, and $\alpha_i(k) > 0$ for all $k_1 \leq k \leq k_2 - 1$.
Note that each $k \in [K]$ belongs to the interval defined by a unique element $(k_1, k_2; i) \in \cal{S}_i$.
In words, $k_1$ and $k_2$ determine the maximal contiguous strip of  indices such that $\alpha_i(k) > 0$.
From \eqref{cpt_sys_kkt4}, $\alpha_i(k) > 0$ implies $\sum_{t=1}^T P_{it} z_{it}(k) =  \sum_{t=1}^T P_{it} z_{it}({k+1})$.

%\begin{claim}
%\label{cl: alpha_pos_exact_match}
%We will show that there is in fact an optimal solution where $\alpha_i(k) > 0$ implies $z_{it}^k = z_{it}^{k+1}$ for all $t \in [T]$.
%\end{claim}
% To see this, suppose $\tilde z$ is an optimal solution to SYS-CPT-K-R and $\bar P_{i}(\tilde z_i(k)) = \bar P_{i}(\tilde z_i^{k+1})$, then consider the allocation $z$ such that 
% $$z_i(k) = z_i^{k+1} = \frac{\tilde z_i(k) +  \tilde z_i^{k+1}}{2},$$
% and $z$ is same as $\tilde z$ everywhere else.
% Note that $z$ is also an optimal solution to SYS-CPT-K-R.


Thus, corresponding to any element $(k_1, k_2; i) \in \cal{S}_i$ we have a common vector $z_{i, \bullet}^* = (z_{it}^*)_{t \in [T]}$ such that $z_{i, \bullet}^* = z_{i, \bullet}(k)$ for all $k_1 \leq k \leq k_2$.
From \eqref{cpt_sys_kkt1}, we have
\begin{align}
    h_i(k) P_{it} -\lambda_i(k) - \frac{\mu_t}{k} = P_{it} (\alpha_i({k-1}) - \alpha_i({k})),
\end{align}
for all $z_{i,t}^* > 0$.
Telescoping over $k_1 \leq k \leq k_2 + 1$, we get
\begin{align}
    P_{it}(\sum_{k = k_1}^{k_2} h_i(k)) = \sum_{k = k_1}^{k_2}\lambda_i(k) + \sum_{k = k_1}^{k_2}\frac{\mu_{t}}{k}.
\end{align}

Suppose there are more than one tiers $t$, say $t \neq t'$, for which $z_{it}^* > 0$, the we get
\begin{align}
    (P_{i t} - P_{i t'}) (\sum_{k = k_1}^{k_2} h_i(k)) = (k_2 - k_1 + 1) \frac{\mu_{t} - \mu_{t'}}{K}.
\end{align}

Now using a similar argument as outlined above theorem \ref{thm:gap_bound}, we get that there are at most $T$ elements in $\cup_{i} \cal{S}_i$ such that the common vector $z_i^*$ has more than one non-zero entries.
Let $\cal{T}$ denote the set of all such elements.
We have 
\begin{equation}
\label{eq: sparsity}
    |\cal{T}| \leq T,
\end{equation} 
and
thus, we get the required sparsity result.
We will now use it to bound the gap coming from approximation \eqref{eq: cpt_approx}.



\begin{theorem}\label{thm:cpt_gap_bound}
Let $V^*$ and $V^R$ be the optimal objectives of the problem in SYS-CPT-K and SYS-CPT-K-R, respectively. 
We have,
\begin{equation}
V^* \geq \left(1 - \frac{T(\max_i J_i)}{\min_t M_t}\right) V^R.
\end{equation}  
\end{theorem}


\begin{proof}
%Suppose the resource allocation matrix $\x^R \in \R^{N\times T}$ is $(N+T)$-sparse (which holds in a generic case as discussed earlier).
%due to the condition in Eq. \eqref{sys_kkt1}. 
% Furthermore, no two users can get partial resources across the same two tiers
Let $\z^R$ be an optimal resource allocation $\z^R$ for SYS-CPT-K-R.
Suppose $(k_1, k_2, i) \in \cal{T}$ corresponding to $\z^R$. 
That is, user $i$ is getting non-zero resources in slots $m$ and $n$ (and say $m < n$) in alternatives $k_1$ through $k_2$, i.e. $z_{im}(k) > 0, x_{in}(k) > 0, \forall k_1 \leq k \leq k_2$.
Recall that ${z_{i, \bullet}^R(k)}$ are identical for all $k_1 \leq k \leq k_2$.
Consider a user $j$ which is getting positive resources in slot $m$ and alternative $k'$, i.e. $z_{jm}({k'}) > 0$. 

Suppose we redistribute $\epsilon (>0)$ fraction of the job from user $j$ in slot $m$ and alternative $k'$ to user $i$ in slot $m$ and alternatives $k \in [k_1, k_2]$ (equally distributed) and vice versa in slot $n$. 
By the optimality of $\z^R$, we know that this can only decrease the objective function in SYS-CPT-K-R, that is
$$\l(\frac{\sum_{k = k_1}^{k_2} h_i(k)}{k_2 - k_1 + 1}\r)(P_{im} - P_{in})\epsilon - h_j(k)(P_{jm} - P_{jn})\epsilon \leq 0.$$
Then, , we have
\begin{equation}
\label{eq: cpt_relation_P}
\l(\frac{\sum_{k = k_1}^{k_2} h_i(k)}{k_2 - k_1 + 1}\r)(P_{im} - P_{in}) \leq h_j({k'})(P_{jm} - P_{jn}).
\end{equation}

Now, we are ready to prove the theorem. From Eq. \eqref{eq: cpt_value_ineq}, we get that 
$$\frac{V^R - V^*}{V^R} \leq \frac{V^R - \tilde V}{V^R}$$ 
where $\tilde V$ is the objective of SYS-CPT-K at $\tilde \z$ obtained by projecting solution of SYS-CPT-K-R as described in Eq. \eqref{eq: cpt_end_time_def_k_best}, \eqref{eq: cpt_endT_to_cum_prob_k_best}, and \eqref{eq: tilde_q_to_tilde_z}. 


Now, our aim is to upper bound the RHS above to get an upper bound on the gap. 
To that end, we bound the numerator and denominator at each time slot $t\in [T]$. 
Let $V^R_t$ and $\tilde V_t$ be the corresponding utilities obtained only at tier $t\in [T]$, i.e.
\[
    V^R_t := \sum_{i = 1}^N \sum_{k = 1}^K h_i(k) P_{it} z_{it}(k) \quad \text{ and } \quad \tilde V_t := \sum_{i = 1}^N \sum_{k = 1}^K h_i(k) P_{it} \tilde z_{it}(k).
\]
%where $y^R_{it}$ and $\hat y_{it}, \forall i, t,$ are as defined in \eqref{eq: y_R_def} and \eqref{y_hat}, respectively.
Let $\tilde T_i$ be the time at which the job of user $i$ are getting finished according to the resource allocation $\z^R$ as defined in \eqref{eq: cpt_end_time_def_k_best}.

Thus, for time slot $m$, we have
\begin{equation}
\frac{V^R_m - \tilde V_m}{V^R_m} = \frac{\sum_{(k_1, k_2; i) \in \cal{T}_m} \sum_{k = k_1}^{k_2} h_i(k)(P_{im} - P_{i \tilde T^k_i}){z^R_{im}(k) } }{\sum_{j=1}^N \sum_{k = 1}^{K} P_{jm} {z_{jm}^R(k)}},
\end{equation}   
where $\cal{T}_m$ is the set of elements $(k_1, k_2; i) \in \cal{T}$ for which $0 < {z^R_{im}(k)} < J_i$, for $k_1 \leq k \leq k_2$. 
%Formally, $S_t := \{i\in [N], 0 < x^R_{it} < J_i\}$. 
%Also, $\tau_i$ is the time at which jobs of user $i$ are getting finished, that is, $\sum_{t=0}^{\tau_i} x_{it} = J_i$ (in case user $i$'s jobs are not getting completely finished, $\tau_i = T+1$ and $P_{i\tau_i} = 0$). 
We can further write
\begin{align}
\frac{V^R_m - \tilde V_m}{V^R_m} 
&\leq \sum_{(k_1, k_2;i) \in \cal{T}_m}
\frac{ (\sum_{k=k_1}^{k_2} h_i(k))  (P_{im} - P_{i \tilde T^k_i}) {z^R_{it}(k)}}{\sum_{j=1}^N \sum_{k = 1}^{K} h_j(k) (P_{jm} - P_{j \tilde T^k_i}) {z^R_{jt}(k)}}\\
&\leq \sum_{(k_1, k_2;i) \in \cal{T}_m}
\frac{ (\sum_{k=k_1}^{k_2} h_i(k))  (P_{im} - P_{i \tilde T^k_i}) {z^R_{it}(k) }}{\sum_{j=1}^N \sum_{k = 1}^{K} \frac{\sum_{k=k_1}^{k_2} h_i(k)}{k_2 - k_1 +1}  (P_{im} - P_{i \tilde T^k_i}) {z^R_{jt}(k)}},
\end{align}
where the last inequality uses Eq. \eqref{eq: cpt_relation_P}. 
Now, since at time $m$, user $i$ is getting fractional resources, it implies that the system is operating at full capacity, that is 
\[
  \frac{1}{K}\sum_{j=1}^N \sum_{k = 1}^K {z^R_{jt}(k)} = M_t.  
\] 
Hence, we get
\begin{align}
\frac{V^R_t - \tilde V_t}{V^R_t} \leq \sum_{(k_1, k_2;i) \in \cal{T}_m} \frac{K {z^R_{it}(k)} }{(k_2 - k_1 + 1) M_t} \leq \sum_{(k_1, k_2;i) \in \cal{T}_m} \frac{\max_i(J_i)}{M_t},
\end{align}
where the last inequality uses the fact that ${z^R_{it}(k)} \leq \max_i(J_i)$ and $k_2 - k_1 + 1 \leq K$. 
Also, since $\cal{T} \leq T$, we get
\begin{align}
\frac{V^R_t - \tilde V_t}{V^R_t} \leq \frac{T\max_i(J_i)}{M_t} \leq \frac{T\max_i(J_i)}{\min_t M_t}.
\end{align}
Thus,
\begin{align}
V^R - V^* \leq V^R - \tilde V = \sum_{t=1}^T (V^R_t - \tilde V_t) \leq \frac{T\max_i(J_i)}{\min_t M_t}\sum_{t=1}^T V^R_t = \frac{T\max_i(J_i)}{\min_t M_t} V^R,
\end{align}
Rearranging, we get
$$V^* \geq \left(1 - \frac{T(\max_i J_i)}{\min_t M_t}\right) V^R,$$
which proves the desired result.
\end{proof}



% {\bf Proof Sketch of Claim~\ref{cl: alpha_pos_exact_match}:}
% We will decompose the problem SYS-CPT-K-R into user problems and network problems in order to decouple the the different users.
% Here we will use a different decomposition from the one that we used earlier in section~\ref{sec:analyse}.

% \begin{align}
% \text{\bf\underline{CPT-USER (i)}} \nn \\
% \max_{\z_i(k) \geq 0} ~~~~~&  \sum_{k=1}^{K} h_i(k) \bP_i(\z_{i}^{k}) - \sum_{t = 1}^T \bar \rho_{it} \bar z_{it} \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~  k \in [K], \label{eq: user_cpt_lp_r_1}\\
%  &\frac{1}{K} \sum_{k=1}^K z_{it}^k = \bar z_{it}, ~\forall ~t \in[T],\label{eq: user_cpt_lp_r_2}\\
%  &\bP_i(\z_i^{k}) \geq \bP_i(\z_i^{k+1}), ~\forall ~1 \leq k \leq K-1 \label{eq: user_cpt_lp_r_3}.
% \end{align}

% \begin{align}
% \text{\bf\underline{CPT-NETWORK}} \nn \\
% \max_{\bar z_{it} \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{t = 1}^T \bar \rho_{it} \bar z_{it} \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{i=1}^{N} \bar z_{it}^k \leq M_{t}, ~\forall ~t \in[T],\label{eq: net_cpt_lp_r_2}
% \end{align}

% This decomposition allows us to decouple the preferences of the different users. 
% Note that the preference features of each player, namely, her utility and probability weighting functions, appear in her corresponding CPT-USER problem. And the CPT-NETWORK problem correlates different players' preferences via psuedo prices $\bar \rho_{it}$.
% We will use this decomposition to study the typical lottery-allocation received by a player by analysing the CPT-USER(i) problem.
%\iffalse





==> CPT_uniform_quant.tex <==
%!TEX root = main.tex

\section{Lottery-based Resource Allocation}
\label{sec: CPT_model}

In the previous sections, we focused on the importance of taking into account the delay-sensitivity characteristics of the agents while allocating resources in serverless systems.
The purpose of considering delay-sensitivity characteristics was to distinguish between agents who have different QoS (quality-of-service) requirements based on the delay in the execution of their jobs.
We saw how to allocate resources that would prioritize the customers based on their delay-sensitivity requirements and charge them appropriately.
A potential problem of such market-based pricing scheme is that
if the supply of resources exceeds the demand by a lot, then it might drive the prices high and discourage some of the smaller customers from participating in such markets.
Several service providers use lottery-based allocations to decide which agents to serve next.
As a result, all the customers who are willing to pay the minimum price set by the service provider get a shot at receiving services. 
Such lottery-based provisions, however, give rise to uncertainties in the execution of the jobs or their delay times.
Just as we distinguished between different customers with varying delay-sensitivity, another important criteria for the QoS is the uncertainty in execution of jobs, and different agents have different preferences towards these uncertainties.
In practice, it is common to make provisions in the SLAs (service-level-agreements)
to provide compensation to the customers if a certain fraction of their jobs are not executed in time.
Currently, most service providers have a fixed SLA agreement, but such a "one-size fits all" approach is inefficient.
In this section, we show that we can build on our system model to account for such lottery-based allocations.
The concept of utility functions from economics helped us model the delay-sensitivity of the customers.
Now again, economics offers us the notion of probabilistic-sensitivity to model customers' preferences towards uncertainties.


Suppose the uncertain completion time for user $i$ is given by the lottery
\begin{equation}
\label{eq: lottery_form}
     L_i = \{(p_i^1, y_i^1), \dots, (p_i^K, y_i^K) \},
\end{equation}
where $y_i^k \geq 0, k \in [K]$, are the completion times and $p_i^k$ the corresponding probabilities with which they occur.
We assume the lottery to be exhaustive, i.e. $\sum_{j = 1}^k p_i^j = 1$.
(Note that we are allowed to have $p_i^k = 0$ for some values of $k \in [K]$ and $y_i^k = y_i^{k'}$ for some $k, k' \in [K]$.)
A natural approach to account for such uncertainties is to use expected utility instead of the utility corresponding to any single completion time.
Thus the ``happiness'' of user $i$ under expected utility theory (EUT) for lottery $L_i$ will be given by
$\sum_{k = 1}^K p_i^k U_i(y_i^k).$


We now consider the multi-tier model with $T$ tiers and $N$ users.
Recall that $\tau_t$ denotes the end time of tier $t$ and $U_i^t = U_i(\tau_t)$.
Let $q_{it}$ denote the probability that user $i$'s jobs are completed by tier $t$.
Let $p_{it} := q_{it} - q_{i(t-1)}$ denote the probability that user $i$'s jobs are allocated in tier $t$.
Suppose we ask that the cloud capacity constraints are satisfied in expectation.
Then this condition can be written as the constraint $\sum_{i = 1}^N p_{it} J_i \leq M_t$, for all $t$.
The problem of maximizing expected utility with a probabilistic allocation of resources to users is given by
\begin{align}
\text{\bf\underline{SYS-EU}} \nn \\
\max _{p_{it} \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{t=1}^{T} p_{it} U_{i}^t \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} p_{i t} \leq 1, \forall i \in[N]\\
 & \sum_{i=1}^{N} p_{i t} J_{i} \leq M_{t}, \forall t \in[T].
\end{align}
%Here, the system constraints are satisfied on average.


We now observe that SYS-EU is exactly same as SYS-LP with the transformation $x_{it} = p_{it} J_i$.
Since we know how to solve the problem SYS-LP, we get the solution for SYS-EU.
Further, the sparsity of the solution $\x$ to SYS-LP (see Theorem~\ref{thm:gap_bound}), shows that for most of the users we have a lottery $L_i$ that allocates resources in a specific tier with probability $1$.
Thus, \emph{for most of the users, we assign them deterministic lotteries under EUT}.


Such an allocation scheme would result in discouraging the users who have lower willingness-to-pay as mentioned before.
Consider a user whose willingness-to-pay is $\$1$ to get her job completed in $1$ sec.
Suppose the market price is $\$1.5$ for job completion within $1$ sec.
It is possible that this user is ready to pay $\$0.2$ to get a $10\%$ chance of having her job completed in $1$ sec.
Note that this behavior is different from EUT predictions.
In fact, it has been observed through several empirical studies that individuals often do not behave according to EUT and display varying degrees of sensitivity to probabilities.
Lotteries provide a way to capture such customers in the market.
%In this section, we generalize our system model to consider probabilit
The correct model to consider to analyse this phenomenon is cumulative prospect theory (CPT) \cite{tversky1992advances}, a generalization of expected utility, and one of the leading decision theory models.
It allows us to capture the probabilistic-sensitivity of the customers.



We now describe the CPT model that we use to measure the ``happiness'' derived by each player from her lottery (for more details see~\cite{wakker2010prospect}). 
Suppose an agent faces a lottery $L_i$ as shown in \eqref{eq: lottery_form}.
%$$L = \{(p^1, y^1), \dots, (p^k, y^k) \},$$
%where $y_j \in \bbR^+$ are the end times and $p_j$ the corresponding probabilities with which they occur.
%We assume the lottery to be exhaustive, i.e. $\sum_{j = 1}^k p^j = 1$.
%
%It is a generalization of the expected utility theory model (EUT) \citep{von1945theory} of choice under risk, 
%and a special case of cumulative prospect theory (CPT) \citep{tversky1992advances}.
Each player $i$ is associated with a utility function
%\footnote{
%The value function in RDU is generally defined on $\bbR$. However, since we will be dealing only with nonnegative throughputs, we restrict it to $\bbR_+$.
%}
$u_i : \bbR_+ \to \bbR_+$ 
as before, 
and a probability weighting function $w_i : [0,1] \to [0,1]$ that is continuous, 
%\footnote{
%The continuity assumption for the probability weighting function can be relaxed. Discontinuities at $0$ and $1$ are empirically interesting 
%(for more on the phenomenon of ignorance at end points see 
%\citep{kahneman1979prospect}. 
%}
strictly increasing and satisfies $w_i(0) = 0$ and $w_i(1) = 1$. 



For the prospect $L_i$, let $\pi_i : [K] \to [K]$ be a permutation such that
\begin{equation}
	\label{eq: pi_order_1}
	U_i(\tilde y_i^1) \geq U_i(\tilde y_i^2) \geq  \dots \geq U_i(\tilde y_i^k),
\end{equation}
and
\begin{equation}
	\label{eq: pi_order_2}
	\tilde y_i^k = y_i^{\pi_i(k)} \mbox{ for all } k \in [K].
\end{equation}
This is equivalent to the ordering 
\[
    \tilde y_i^1 \leq \tilde y_i^2 \leq  \dots \leq \tilde y_i^k,
\]
since the utility function $U_i(\cdot)$ is assumed to be decreasing.
The prospect $L_i$ can equivalently be written as
\[
	L_i = \{(\tilde p_i^1, \tilde y_i^1); \dots ; (\tilde p_i^K, \tilde y_i^K)\},
\]
where $\tilde p_i^k := p_i^{\pi_i(k)}$ for all $k \in [K]$.
The \emph{CPT value} of prospect $L_i$ for the agent is evaluated using the utility function $U_i(\cdot)$ and the probability weighting function $w_i(\cdot)$ as follows:
\begin{equation}
\label{eq: RDU_formula}
	V_i(L) := \sum_{k = 1}^{K} d_i^{k}(p_i,\pi_i)U_i(\tilde y_i^k),
\end{equation}
where $d_i^{k}(p_i,\pi_i)$ are the \emph{decision weights} given by $d_i^1(p_i,\pi_i) := w_i(\tilde p^1)$ and
\begin{align*}
	d_i^{k}(p_i,\pi_i) := w_i(\tilde p_i^1 + \dots + \tilde p_i^k) - w_i(\tilde p_i^1 + \dots + \tilde p_i^{k - 1}),
\end{align*}
for $1 < k \leq K$.
Although the expression on the right in equation \eqref{eq: RDU_formula} depends on the permutation $\pi_i$, one can check that the formula evaluates to the same value $V_i(L_i)$ as long as $\pi_i$ satisfies \eqref{eq: pi_order_1} and \eqref{eq: pi_order_2}. 
The CPT value of prospect $L_i$, can equivalently be written as
\[
	V_i(L_i) = \sum_{k = 1}^{K} w_i\big(\sum_{s = 1}^{k} \tilde p_i^s\big ) \l[ U_i(\tilde y_i^k) - U_i(\tilde y_i^{k + 1}) \r],
\]
where $\tilde y_i^{K+1} := 0$.
Thus the worst end time $\tilde y_i^{K}$ is weighted by $w_i(1) = 1$, and every increment in the value of the allocations, $U_i(\tilde y_i^k) - U_i(\tilde y_i^{k + 1}), \forall k \in [K -1]$, is weighted by the probability weighting function of the probability of receiving an allocation at least equal to $\tilde y_i^k$.

Some example of weighing functions are provided in Figure \ref{fig:cpt_weighing}.
\sph{@Vipul It would be nice to have plots for different values of $\gamma_i$ in the same figure.}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[scale=0.6]{tex_figs/cpt1.pdf}
        \caption{ $w_{i}^{\pm}(p)=\exp \left\{-(-\ln p)^{\gamma_{i}}\right\}, \gamma_i=0.5$}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[scale=0.6]{tex_figs/cpt2.pdf}
        \caption{  $w_{i}\left(p_{i}\right)=\frac{p_{i}^{\gamma_{i}}}{\left(p^{\gamma_{i}}+(1-p)^{\gamma_{i}}\right)^{1 / \gamma_{i}}}, \gamma_{i}=0.5$}
    \end{subfigure}
    \caption{Utility and price paid by a randomly chosen user}
\label{fig:cpt_weighing}
\end{figure*} 

%Now, let us define $q_{i t}=\sum_{\tau=1}^{t} p_{i \tau}$ as the cumulative probabilities and let $w_i(\cdot)$ as the weighing function (see Fig. \ref{fig:cpt_weighing} for examples). 
Let us now consider the multi-tier based model.
Recall that the difference in the utilities of job completion in tiers $t$ and $t+1$ is given by $u_{it} = U_i^t - U_i^{t+1}$.
Then, the CPT based system problem is given by
\begin{align}
\text{\bf\underline{SYS-CPT}} \nn \\
\max _{p_{it}, q_{it} \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{t=1}^{T} w_{i}\left(q_{i t}\right) u_{i t} \label{eq: sys_cpt_0}\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} p_{i t} \leq 1, \forall i \in[N]\label{eq: sys_cpt_1}\\
 & \sum_{i=1}^{N} p_{i t} J_{i} \leq M_{t}, \forall t \in[T],\label{eq: sys_cpt_2}\\
 & q_{i t}=\sum_{\tau=1}^{t} p_{i \tau}, ~\forall~ i \in[N], t \in[T].
\end{align}
%where $u_{i t}=U_{i}^t-U_{i}^{t+1}$.



\sph{Include a discussion on the non-convexity of the problem SYS-CPT in general. @Vipul Can we include some results from simulation to show that there are several local optima and in general it is hard to find the optimum?}


We now use the discretization trick introduced in \cite{phade2019optimal} to solve SYS-CPT approximately.
Fix an integer $K > 0$.
We restrict our attention to solutions where
\[
    p_{it}, q_{it} \in \l\{\frac{k}{K}: 0 \leq k \leq K \r\} =: \Delta.
\]
Thus, we allow only the probabilities belonging to the discretized mesh $\Delta$.
As $K \to \infty$, we get better approximations to SYS-CPT.
However, there is a practical motivation to keep $K$ limited.
From a behavioral perspective, people often do not comprehend small differences in probability.
For this reason, it is useful to restrict $K$ (for example $K \leq 100$).
Let us call this discretized version of SYS-CPT as SYS-CPT-K.

{\bf A richer problem formulation:}
We now give a richer problem formulation that would help us solve the above discretized version of SYS-CPT.
Suppose the cloud provider achieves a lottery implementation through a scheme as follows: 
The scheduler implements with equal probability one of the $K$ allocation schemes $\x^k := [x_{it}^k], i \in [N], t \in [T]$, for $k \in [K]$.
Let $[K]$ denote the set of \emph{alternatives}.
For alternative $k$, the job end time for user $i$ is given by
\begin{equation*}
%\label{eq: end_time_def}
    T_i^k := \min \{t \in [T] : \sum_{s = 1}^t x_{is}^k \geq J_i \},
\end{equation*}
Thus the probability that user $i$'s jobs are completed by the end of tier $t$ is given by
\[
    q_{it} = \frac{|\{k: T_i^k \leq t \}|}{K},
\]
and the lottery faced by user $i$ is given by
\begin{align*}
    L_i = \{(p_{i1}, \tau_1); \dots; (p_{iT}, \tau_T)\},
\end{align*}
where $p_{it} = q_{it} - q_{i(t-1)}$.
The CPT value of this lottery is
\begin{align}
\label{eq: CPT_val_1}
    V_i(L_i) = \sum_{t = 1}^T w_i(q_{it}) u_i^t.
\end{align}
This lottery can equivalent be written as
\begin{align*}
    L_i = \{({1}/{K}, \tau_{T_i^1});\dots;({1}/{K}, \tau_{T_i^K})\}.
\end{align*} 
Note that in this formulation the end times can appear repeatedly, but the total probability of any particular end time is same in both the formulations.
It is easy to verify that CPT value formula is invariant under such equivalent representations.
Also note that the end times in the second formulation are not ordered.
Let $\pi_i: [K] \to [K]$ be a permutation such that
\[
    {\tilde T_i^1} \leq {\tilde T_i^2} \leq  \dots \leq {\tilde T_i^K},
\]
where $\tilde T_i^k = T_i^{\pi_i(k)}$.
Then the CPT value of user $i$ for lottery $L_i$ is given by
\begin{align}
\label{eq: CPT_value_2}
     V_i(L_i) = \sum_{k = 1}^K h_i^k U_i^{\tilde T_i^k}.
\end{align}
where $h_i^k := w_i(k/K) - w_i((k-1)/K)$ for $k \in [K]$.
Note that the two formulas for the CPT value in \eqref{eq: CPT_val_1} and \eqref{eq: CPT_value_2} are equivalent.
Also note that if $w_i(\cdot)$ is an identity function (as in the EUT setting), then $h_i^k = 1/K$, and the corresponding CPT value is simply the average of the utility from all alternatives. 
%
% Note that when $w_i(0) = 0 ~\forall ~i\in [N]$, the objective in EU-CPT can be equivalently written as
% $$\max _{q_{i t} \geq 0} \sum_{i=1}^{N} \sum_{t=1}^{T} \left(w_{i}q_{it} - w_{i}q_{i(t-1)}\right) U_{i}^t.$$
%
% Let us consider an alternate formulation of EU-CPT, where the cloud provider has $K$ alternatives, with the $k$-th alternative corresponding to a resource allocation matrix $\x^k\in \R^{N\times T}, k\in [K],$ according to which the $N$ users are allocated resources across $T$ tiers. Now, instead of optimizing over cumulative probabilities ($q_{it}$'s), let us optimize over the $K$ alternatives, and hope that the resulting problem will be convex.
%
% Also, let us define the incremental CPT weightings as
% $$ h_i^k = w_i\l(\frac{k}{K}\r) - w_i\l(\frac{k-1}{K}\r) ~\forall ~k \in [K], i\in [N].$$
%


We now use the relaxation trick as in the previous section.
We approximate the utility for user $i$ corresponding to alternative $k$ as follows:
\begin{align}
\label{eq: cpt_approx}
    U_i^{T_i^k} \approx \sum_{t = 1}^T \frac{x_{it}^k U_i^t}{J_i}.
\end{align}
Note that when $(x_{it}^k, t \in [T])$ is $1$-sparse with that non-zero entry equal to $J_i$, the above approximation is exact.
With this relaxation our objective can be written as
\[
    \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\x_{i}^{\pi_i(k)}),
\]
where $\bP(\x_{i}^k) = \sum_{t=1}^T x_{it}^k P_{it} = \sum_{t=1}^T x_{it}^k U_i^t/J_i$ and the permutation $\pi_i(k)$ is such that
\begin{equation}
\label{eq: pi_bar_P_ineq_x}
    \bP_i(\x_i^{\pi_i(1)}) \geq \bP_i(\x_i^{\pi_i(2)}) \geq \cdots \geq \bP_i(\x_i^{\pi_i(K)}),
\end{equation}
for all $i$.



Corresponding to allocations $\x^k, \forall k \in [K]$ and permutations $\pi_i, \forall i \in [N]$, let $z_{it}^k := \x_{it}^{\pi_i(k)}$ be a $|T|$-dimensional column vector, for $i \in [N], k \in [K]$.
With this notation, the objective function can be written as
\begin{equation}
    \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\z_i^k),
\end{equation}
and the inequalities~\eqref{eq: pi_bar_P_ineq_x} take the form
\begin{equation}
    \bP_i(\z_i^1) \geq \bP_i(\z_i^2) \geq \cdots \geq \bP_i(\z_i^K),
\end{equation}
for all $i$.

Strictly speaking, such a scheme in our richer problem formulation is feasible iff each of the alternatives is feasible, i.e. 
\begin{equation}
\label{eq: feasibility_hard_constraint}
    \sum_{i = 1}^N x_{it}^k \leq M_t
\end{equation}
for all $t, k$. However, we will use this richer formulation only as an intermediate step to solve the discretized SYS-CPT problem (namely, SYS-CPT-K) where we are interested in the implementations that feasible in expectation. Hence we will, instead, consider the constraint 
\begin{equation}
    \frac{1}{K} \sum_{k = 1}^K \sum_{i = 1}^N x_{it}^k  \leq M_t, \forall t \in [T].
\end{equation}

This motivates the following relaxed system problem:
\begin{align}
\text{\bf\underline{SYS-CPT-K-R}} \nn \\
\max _{\z^k \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\z_{i}^{k}) \label{eq: sys_cpt_lp_r_0}\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K], \label{eq: sys_cpt_lp_r_1}\\
 &\frac{1}{K} \sum_{k=1}^K\sum_{i=1}^{N} z_{it}^k \leq M_{t}, ~\forall ~t \in[T],\label{eq: sys_cpt_lp_r_2}\\
 &\bP_i(\z_i^{k}) \geq \bP_i(\z_i^{k+1}), ~\forall~i \in [N], ~\forall ~1 \leq k \leq K-1. \label{eq: sys_cpt_lp_r_3}
\end{align}


Notice that the problem SYS-CPT-K-R is an LP problem.
% Besides, the value of the problem SYS-CPT-K-R is equal to the value of the problem SYS-CPT-K-2.
% (Further details relating the primal and dual values the problems SYS-CPT-K-2, SYS-CPT-3 and SYS-CPT-R can be found in \cite{phade2019optimal}).
%Let us now compare the constraint \eqref{eq: sys_cpt_1} with \eqref{eq: sys_cpt_lp_r_1} and the contraint \eqref{eq: sys_cpt_2} with \eqref{eq: sys_cpt_lp_r_2}.
Suppose $\tilde p_{it}, \tilde q_{it} \in \Delta$ is a feasible solution to the SYS-CPT-K problem.
Then, let us construct $\tilde z$ as follows: for player $i$, let 
\begin{equation}
     \tilde z_{it}^k = \begin{cases}
        J_i, &\text{ if } q_{i(t-1)}K < k \leq q_{it},\\
        0, &\text{ otherwise,}
    \end{cases}
\end{equation}
for all $t, k$.
One can verify that $\tilde z$ is a feasible solution to SYS-CPT-K-R, and the the objectives \eqref{eq: sys_cpt_lp_r_0} and \eqref{eq: sys_cpt_0} match exactly.
This is because the allocations $z_i^k$ are $1$-sparse with the non-zero entry equal to $J_i$, and hence
the approximation in \eqref{eq: cpt_approx} is exact.
   


On the other hand, if we take
\[
    p_{it} = \frac{1}{K} \sum_{k = 1}^K z_{it}^k,
\]
then, we observe that a feasible solution $z_{it}^k$ to SYS-CPT-K-R gives rise to a feasible solution to SYS-CPT.
\sph{@Vipul We should simulate and compare these two solutions.}


In Appendix~\ref{sec: hard_const_relax}, we set up the richer problem formulation and require that the \emph{hard feasibility constraints} hold as in ~\eqref{eq: feasibility_hard_constraint}. However, this problem is NP-hard because it requires an optimal permutation $\pi_i(k)$ to allocate the lotteries.
Treating the permuations as matrices and relaxing them to be doubly stochastic matrices we get SYS-CPT-R.
Besides, as proved in \cite{phade2019optimal}, the dual value of the richer problem formulation with hard costraints is equal to the value of the problem SYS-CPT-K-R.


In the following, we will establish the sparsity of the optimal solution $z$ to SYS-CPT-K-R, and use this to bound the gap between the optimal solutions of SYS-CPT-K and SYS-CPT-K-R.
But before that, let us take a closer look at the problem SYS-CPT-K-R.




% With this interpretation in terms of $[K]$ alternatives, we get the following problem:
% \begin{align}
% \text{\bf\underline{SYS-CPT-K}} \nn \\
% \max_{\substack{
% \x^k \geq 0,\forall k,\\
% \pi_i,\forall i,\\
% T_i^k, \tilde T_i^k, \forall i,k 
% }} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k U_i^{\tilde T_i^k} \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} x_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K],\\
%  & \sum_{i=1}^{N} x_{it}^k \leq M_{t}, ~\forall ~t \in[T], k \in [K],\\
%  & T_i^k := \min \{t \in [T] : \sum_{s = 1}^t x_{is}^k \geq J_i \}, ~\forall~i \in [N], k \in [K],\\
%  & \tilde T_i^k = T_i^{\pi_i(k)},~\forall~i \in [N], k \in [K],\\
%  & {\tilde T_i^1} \leq {\tilde T_i^2} \leq  \dots \leq {\tilde T_i^K}, ~\forall i \in [N].
% \end{align}

% We now use the relaxation trick as in the previous section.
% We approximate the utility for user $i$ corresponding to alternative $k$ as follows:
% \begin{align}
% \label{eq: cpt_approx}
%     U_i^{T_i^k} \approx \sum_{t = 1}^T \frac{x_{it}^k U_i^t}{J_i}.
% \end{align}
% Note that when $(x_{it}^k, t \in [T])$ is $1$-sparse with that non-zero entry equal to $J_i$, the above approximation is exact.
% With this relaxation our problem can be written as
% \begin{align}
% \text{\bf\underline{SYS-CPT-K-1}} \nn \\
% \max _{\x^k \geq 0, \pi_i} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\x_{i}^{\pi_i(k)}) \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} x_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K],\\
%  & \sum_{i=1}^{N} x_{it}^k \leq M_{t}, ~\forall ~t \in[T], k \in [K],
% \end{align}
% where $\bP(\x_{i}^k) = \sum_{t=1}^T x_{it}^k P_{it} = \sum_{t=1}^T x_{it}^k U_i^t/J_i$ and the permutation $\pi_i(k)$ is such that
% $$ \bP_i(\x_i^{\pi_i(1)}) \geq \bP_i(\x_i^{\pi_i(2)}) \geq \cdots \geq \bP_i(\x_i^{\pi_i(K)}).$$
% Note that the non-convex function $w_i(\cdot)$ is represented in the relaxed problem as constants $h_i^k$ due to discretization. However, the relaxed problem is still NP-hard since it requires an optimal permutation $\pi_i(k)$ to allocate the lotteries (we will discuss more on how to allocate lotteries with this formulation later). 

% We now further relax the above problem by using the trick from \cite{phade2019optimal}.
% This involves re-writing the problem by representing the permutations as a permutation matrix and relaxing them to doubly stochastic matrices.
% We now give the details of this transformation.
% %This gives rise to the following problem (see~\cite{phade2019optimal} for details of this transformation):
% Corresponding to allocations $\x^k, \forall k \in [K]$ and permutations $\pi_i, \forall i \in [N]$, let $z_{it}^k := \x_{it}^{\pi_i(k)}$ be a $|T|$-dimensional column vector, for $i \in [N], k \in [K]$, and let $S_i$ be the $K \times K$ matrix given by $S_i(s,t) = 1$ if $\pi_i(t) = s$ and $S_i(s,t) = 0$ otherwise, for $s,t \in [K], i \in [N]$.
% Note that $S_i$ is the permutation matrix corresponding to the permutation $\pi_i^{-1}$~(i.e. inverse of the permutation $\pi_i$).
% Note that $S_i$ is also a doubly stochastic matrix.
% Let $\Omega_K$ denote the set of all $K \times K$ doubly stochastic matrices, and
% let $\Omega_K^*$ denote the set of all $K \times K$ permutation matrices.
% Also note that the allocations $\x^k, \forall k \in [K]$ and the permutations $\pi_i, \forall \in [N]$ are uniquely defined by $\z := (z_{it}^k, i \in [N], t \in [T], k \in [K])$, and $S_i, i \in [N]$.
% Let $\z_i^k := (z_{it}^k, t \in [T])$ and $\z_{it} := (z_{it}^k, k \in [K])$ denote column vectors.
% Let $\1$ denote a column vector of dimension $K$.
% The problem SYS-CPT-K-1 can equivalently be written as follows:
% \begin{align}
% \text{\bf\underline{SYS-CPT-K-2}} \nn \\
% \max_{\z \geq 0, S_i \in \Omega_K^*} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\z_i^k) \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K],\\
%  & \sum_{i=1}^{N} S_i \z_{it} \leq M_{t} \1, ~\forall ~t \in[T],\\
%  &\bP_i(\z_i^1) \geq \bP_i(\z_i^2) \geq \cdots \geq \bP_i(\z_i^K).
% \end{align}

% We now relax the constraint $S_i \in \Omega_K^*$ to be $S_i \in \Omega_K$.
% This gives us the following problem:
% \begin{align}
% \text{\bf\underline{SYS-CPT-K-3}} \nn \\
% \max_{\z \geq 0, S_i \in \Omega_K} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\z_i^k) \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~ i \in[N],\\
%  & \sum_{i=1}^{N} S_i \z_{it} \leq M_{t} \1, ~\forall ~t \in[T],\label{eq: sys_cpt_k_3}\\
%  &\bP_i(\z_i^1) \geq \bP_i(\z_i^2) \geq \cdots \geq \bP_i(\z_i^K).
% \end{align}

% Notice that the constraint $\sum_{i=1}^{N} S_i \z_{it} \leq M_{t}$ implies that 
% \[
%     \frac{1}{K} \sum_{k=1}^K \sum_{i=1}^{N} z_{it}^k = \frac{1}{K} \sum_{i=1}^{N} \1^T S_i z_{it} \leq \1^T M_t \1 \leq M_t.
% \]
% If we replace constraint \eqref{eq: sys_cpt_k_3} by the above condition we get
% \begin{align}
% \text{\bf\underline{SYS-CPT-K-R}} \nn \\
% \max _{\z^k \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\z_{i}^{k}) \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K], \label{eq: sys_cpt_lp_r_1}\\
%  &\frac{1}{K} \sum_{k=1}^K\sum_{i=1}^{N} z_{it}^k \leq M_{t}, ~\forall ~t \in[T],\label{eq: sys_cpt_lp_r_2}\\
%  &\bP_i(\z_i^{k}) \geq \bP_i(\z_i^{k+1}), ~\forall~i \in [N], ~\forall ~1 \leq k \leq K-1. \label{eq: sys_cpt_lp_r_3}
% \end{align}




\sph{Let $w_i^*: [0,1] \to [0,1]$ be the minimum concave function that dominates $w_i$, i.e. $w_i^*(p_i) \geq w_i(p_i)$ for all $p_i \in [0,1]$. Let $p_i^* \in [0,1]$ be the smallest probability such that $w_i^*(p_i)$ is linear over the interval $[p_i^*, 1]$.
Include a subsection showing that the lowest alternative allocations for any player $i$, $z_t^k$ are identical for all $k \geq k_i^*$, where $k_i^*$ is the smallest integer greater equal $p_i^*$.}

%Here, we relaxed the constraints such that the system and user job constraints are satisfied on average (as in the EU problem). Now, the idea is to show that the overall CPT utility of the system through the three problems is almost the same, that is, EU-CPT-R2 $\approx$ EU-CPT-R $\approx$ EU-CPT

{\bf Sparsity of optimal lottery allocation:}
Let $\lambda_i^k, \mu^t, \alpha_i^k$ denote the dual variables corresponding to the constraints \eqref{eq: sys_cpt_lp_r_1}, \eqref{eq: sys_cpt_lp_r_2}, and \eqref{eq: sys_cpt_lp_r_3}.
The complementary slackness conditions for the SYS-CPT-K-R problem are:
\begin{align}
\label{cpt_sys_kkt1} 
h_{i}^k P_{it} - \lambda_i^k - \frac{\mu_t}{k} + P_{it} (\alpha_i^k - \alpha_i^{k-1})
&\begin{cases}
= 0, & \text{ if } z_{it}^k > 0,\\
\geq 0, & \text{ if } z_{it}^k = 0,
\end{cases}
\quad \quad \forall i, t,\\
\label{cpt_sys_kkt2} 
\sum_{t = 1}^T \sum_{k=1}^{K} z_{it}^k 
&\begin{cases}
= J_i, & \text{ if } \lambda_i^k > 0,\\
\leq J_i, & \text{ if } \lambda_i^k = 0,
\end{cases}
\quad \quad ~\forall i,\\
\label{cpt_sys_kkt3}
\frac{1}{K} \sum_{i=1}^N \sum_{k=1}^{K} z_{it}^k 
&\begin{cases}
= M_t, & \text{ if } \mu_t > 0,\\
\leq M_t, & \text{ if } \mu_t = 0,
\end{cases}
\quad \quad ~~~\forall t,\\
\label{cpt_sys_kkt4}
\sum_{t=1}^T P_{it} z_{it}^k -  \sum_{t=1}^T P_{it} z_{it}^{k+1} 
&\begin{cases}
= 0, & \text{ if } \alpha_i^k > 0,\\
\geq 0, & \text{ if } \alpha_i^k = 0,
\end{cases}
\quad \quad ~~~\forall i, k.
\end{align}
Now observe that $\alpha_i^0 = \alpha_i^K = 0$ for all $i$.
Consider the set $\cal{S}_i$ comprising of all tuples $(k_1, k_2)$ such that $0 < k_1 \leq k_2 < K$, $\alpha_i^{k_1 - 1} = \alpha_i^{k_2} = 0$, and $\alpha_i^k > 0$ for all $k_1 \leq k \leq k_2 - 1$.
Note that each $k \in [K]$ belongs to the interval defined by a unique tuple $(k_1, k_2) \in \cal{S}_i$.
In words, $k_1$ and $k_2$ determine the maximal contiguous strip of  indices such that $\alpha_i^k > 0$.
From \eqref{cpt_sys_kkt4}, $\alpha_i^k > 0$ implies $\sum_{t=1}^T P_{it} z_{it}^k =  \sum_{t=1}^T P_{it} z_{it}^{k+1}$.

%\begin{claim}
%\label{cl: alpha_pos_exact_match}
We will show that there is in fact an optimal solution where $\alpha_i^k > 0$ implies $z_{it}^k = z_{it}^{k+1}$ for all $t \in [T]$.
%\end{claim}
To see this, suppose $\tilde z$ is an optimal solution to SYS-CPT-K-R and $\bar P_{i}(\tilde z_i^k) = \bar P_{i}(\tilde z_i^{k+1})$, then consider the allocation $z$ such that 
$$z_i^k = z_i^{k+1} = \frac{\tilde z_i^k +  \tilde z_i^{k+1}}{2},$$
and $z$ is same as $\tilde z$ everywhere else.
Note that $z$ is also an optimal solution to SYS-CPT-K-R.


Thus, corresponding to any tuple $(k_1, k_2) \in \cal{S}_i$ we have a common vector $z_i^* = (z_{it}^*)_{t \in [T]}$ such that $z_i^* = z_{i}^k$ for all $k_1 \leq k \leq k_2$.
From \eqref{cpt_sys_kkt1}, we have
\begin{align}
    h_i^k P_{it} -\lambda_i^k - \frac{\mu_t}{k} = P_{it} (\alpha_i^{k-1} - \alpha_i^{k}),
\end{align}
for all $z_i^* > 0$.
Telescoping over $k_1 \leq k \leq k_2 + 1$, we get
\begin{align}
    P_{it}(\sum_{k = k_1}^{k_2} h_i^k) = \sum_{k = k_1}^{k_2}\lambda_i^k + \sum_{k = k_1}^{k_2}\frac{\mu_{t}}{k}.
\end{align}

Suppose there are more than one tiers $t$, say $t \neq t'$, for which $z_{it}^* > 0$, the we get
\begin{align}
    (P_{i t} - P_{i t'}) (\sum_{k = k_1}^{k_2} h_i^k) = (k_2 - k_1 + 1) \frac{\mu_{t} - \mu_{t'}}{K}.
\end{align}

Now using a similar argument as outlined above theorem \ref{thm:gap_bound}, we get that there are at most $T$ tuples in $\cup_{i} \cal{S}_i$ such that the common vector $z_i^*$ has more than one non-zero entries.
Thus, we get the required sparsity result.
We will now use it to bound the gap coming from approximation \eqref{eq: cpt_approx}.


% {\bf Proof Sketch of Claim~\ref{cl: alpha_pos_exact_match}:}
% We will decompose the problem SYS-CPT-K-R into user problems and network problems in order to decouple the the different users.
% Here we will use a different decomposition from the one that we used earlier in section~\ref{sec:analyse}.

% \begin{align}
% \text{\bf\underline{CPT-USER (i)}} \nn \\
% \max_{\z_i^k \geq 0} ~~~~~&  \sum_{k=1}^{K} h_i^k \bP_i(\z_{i}^{k}) - \sum_{t = 1}^T \bar \rho_{it} \bar z_{it} \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~  k \in [K], \label{eq: user_cpt_lp_r_1}\\
%  &\frac{1}{K} \sum_{k=1}^K z_{it}^k = \bar z_{it}, ~\forall ~t \in[T],\label{eq: user_cpt_lp_r_2}\\
%  &\bP_i(\z_i^{k}) \geq \bP_i(\z_i^{k+1}), ~\forall ~1 \leq k \leq K-1 \label{eq: user_cpt_lp_r_3}.
% \end{align}

% \begin{align}
% \text{\bf\underline{CPT-NETWORK}} \nn \\
% \max_{\bar z_{it} \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{t = 1}^T \bar \rho_{it} \bar z_{it} \nn\\
% % \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
% \text{subject to} ~~~~~& \sum_{i=1}^{N} \bar z_{it}^k \leq M_{t}, ~\forall ~t \in[T],\label{eq: net_cpt_lp_r_2}
% \end{align}

% This decomposition allows us to decouple the preferences of the different users. 
% Note that the preference features of each player, namely, her utility and probability weighting functions, appear in her corresponding CPT-USER problem. And the CPT-NETWORK problem correlates different players' preferences via psuedo prices $\bar \rho_{it}$.
% We will use this decomposition to study the typical lottery-allocation received by a player by analysing the CPT-USER(i) problem.


\subsection{Pricing Mechanisms for Lottery-based Allocation}
Similar to the EU case, we will split the system problem SYS-CPT-K-R into USER and CLOUD problems to learn user utilities by getting feedback from users corresponding to different lotteries. We define the USER problem as 
\begin{align}
\text{\bf\underline{USER (i)}} \nn \\
\max_{\z_i^k \geq 0} ~~~~~& \sum_{t=1}^T \sum_{k=1}^{K} h_i^k \frac{m_{it}^k}{\mu_t}(P_{it} - \mu_t) \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} \frac{m_{it}^k}{\mu_t} \leq \frac{J_i}{K}, ~\forall~  k \in [K], \label{cons:user_jobs}\\
 &\sum_{t=1}^T \frac{m_{it}^k}{\mu_t}P_{it} \geq \sum_{t=1}^T \frac{m_{it}^{k+1}}{\mu_t}P_{it}, ~\forall ~1 \leq k \leq K-1 \label{cons:user_k}.
\end{align}

\begin{align}
\text{\bf\underline{NETWORK}} \nn \\
\max_{\bar z_{it} \geq 0} ~~~~~& \sum_{k=1}^{K}\sum_{i=1}^{N} \sum_{t = 1}^T m_{it}^k \log(z_{it}^k) \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~&\frac{1}{K} \sum_{k=1}^{K}\sum_{i=1}^{N} z_{it}^k \leq M_{t},~\forall ~t \in[T].\label{cons:net_machines}
\end{align}

==> CPTmarket.tex <==
%!TEX root = main.tex


\section{Pricing Mechanisms for Lottery-based Allocation}
\label{sec: cpt_market}


Previously, we assumed that the users' utilities are known at the cloud provider. However, this is not true in general. Here, we design a feedback-based scheme to find the optimal lottery allocation.
Similar to the EU case, we will split the system problem SYS-CPT-K-R into USER and CLOUD problems to learn user utilities by getting feedback from users corresponding to different lotteries. 

To decompose the problem, we define a new variable $\m \in \R^{K\times N\times T}$, which is representative of users' budgets corresponding to different lotteries and different tiers. We define the USER problem as 
\begin{align}
\text{\bf\underline{USER (i)}} \nn \\
\max_{m_i^k \geq 0} ~~~~~& \sum_{t=1}^T \sum_{k=1}^{K} \frac{m_{it}^k}{\mu_t}(h_i^kP_{it} -\delta_k \mu_t) \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} \frac{m_{it}^k}{\mu_t} \leq J_i, ~\forall~  k \in [K], \label{cons:user_jobs}\\
 &\sum_{t=1}^T \frac{m_{it}^k}{\mu_t}P_{it} \geq \sum_{t=1}^T \frac{m_{it}^{k+1}}{\mu_t}P_{it}, ~\forall ~1 \leq k \leq K-1 \label{cons:user_k}.
\end{align}

Given a solution $\m$ to the USER(i) problem, the cloud provider solves the following problem for $\z$: 

\begin{align}
\text{\bf\underline{CLOUD}} \nn \\
\max_{z_{it}^k \geq 0} ~~~~~& \sum_{k=1}^{K}\sum_{i=1}^{N} \sum_{t = 1}^T \delta_k m_{it}^k \log(z_{it}^k) \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{k=1}^{K}\sum_{i=1}^{N}\delta_k z_{it}^k \leq M_{t},~\forall ~t \in[T].\label{cons:net_machines}
\end{align}

\begin{theorem}
\label{thm:decomposition}
There exist equilibrium matrices $\z = (z_{it}^k, i\in [N], t\in [T], k\in [K])$ and $\m = (m_{it}^k, i\in [N], t\in [T], k\in [K])$, and an equilibrium price vector $\bmu = (\mu_t, t\in [T])$ such that
\begin{enumerate}[(i)]
    \item $\m_i = (m_{it}^k, t\in [T], k\in [K])$ solves USER(i), $\forall~ i\in [N],$
    \item $\z = (z_{it}^k, i\in [N], t\in [T], k\in [K])$ solves the CLOUD problem,
    \item $m_{it}^k = z_{it}^k q_t,$ for all $i\in [N], t\in [T], k\in [K]$,
    \item for any $t$, if $\sum_i\sum_k \delta_k z_{it}^k < M_t$, then $q_t = 0$.
\end{enumerate}
Further, if any matrix $\z = (z_{it}^k, i\in [N], t\in [T], k\in [K])$ that is at equilibrium, i.e. has a corresponding matrix $\m$ and a vector $\bmu$ that together satisfy (i), (ii), (iii), and (iv), then $\z$ solves the system problem SYS-CPT-K-R.
\end{theorem}

\begin{proof}
Lagrangian for the USER(i) problem (with $p_{i}^k$ and $\beta_{i}^k$, $i\in[N], k\in[K]$ as dual variables corresponding to the two constraints):
$$L(\m_i, \p_i, \bb_i) = \sum_{k=1}^{K} \frac{m_{it}^k}{\mu_t}(h_i^kP_{it} -\delta_k \mu_t) + \sum_{k=1}^K p_{i}^k\left(J_i - \frac{m_{it}^k}{\mu_t}\right) + \sum_{k=1}^{K-1}\beta_i^k\left(\sum_{t=1}^T \frac{m_{it}^k}{\mu_t}P_{it} - \sum_{t=1}^T \frac{m_{it}^{k+1}}{\mu_t}P_{it}\right).$$

The corresponding KKT conditions are given by 
\begin{align}
\label{cpt_user_kkt1} 
h_{i}^k P_{it} - \lambda_i^k - \delta_k\mu_t + P_{it} (\alpha_i^k - \alpha_i^{k-1})
&\begin{cases}
= 0, & \text{ if } m_{it}^k > 0,\\
\geq 0, & \text{ if } m_{it}^k = 0,
\end{cases}
\quad \quad \forall i, t,\\
\label{cpt_sys_kkt2} 
\sum_{t = 1}^T \frac{m_{it}^k}{\mu_t} 
&\begin{cases}
= J_i, & \text{ if } p_i^k > 0,\\
\leq J_i, & \text{ if } p_i^k = 0,
\end{cases}
\quad \quad ~\forall i,k,\\
\label{cpt_sys_kkt4}
\sum_{t=1}^T \frac{P_{it}}{\mu_t}(m_{it}^k -  m_{it}^{k+1} )
&\begin{cases}
= 0, & \text{ if } \beta_i^k > 0,\\
\geq 0, & \text{ if } \beta_i^k = 0,
\end{cases}
\quad \quad ~~~\forall i, k.
\end{align}

Similarly, for the CLOUD problem, the Lagrangian (with dual variable $q_t, t\in [T]$) can be written as
$$L(\z,\q) = \delta_k m_{it}^k \log(z_{it}^k) + \sum_{t=1}^Tq_t\left(M_t - \sum_{k=1}^{K}\sum_{i=1}^{N}\delta_k z_{it}^k\right)$$

The corresponding KKT conditions are given by 
\begin{align}
\label{cpt_cloud_kkt1} 
m_{it}^k &= q_t z_{it}^k ~~~\forall~~~~ i,t,k,\\
\label{cpt_cloud_kkt2} 
\sum_{i=1}^N \sum_{k=1}^{K} \delta_k z_{it}^k 
&\begin{cases}
= M_t, & \text{ if } q_t > 0,\\
\leq M_t, & \text{ if } q_t = 0,
\end{cases}
\quad \quad ~~~\forall t,
\end{align}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.7]{figs_2param_n100_scale/cpt_util_vs_user_update.pdf}
        \caption{The tracking algorithm eventually achieves optimal utility.}
        \label{fig:2param_cpt_track}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.7]{figs_2param_n100_scale/price_vs_user_budget_first_hour.pdf}
        \caption{The prices set by the cloud provider and the budgets showed by the users converge to the optimal with the tracking algorithm.}
    \end{subfigure}
    \caption{Performance of the tracking-based algorithm.}
\label{fig:2param_cpt}
\end{figure*} 
Now, observe that given a solution $(\z,\lambda,\mu,\alpha)$ to SYS-CPT-K-R and satisfies the corresponding KKT conditions, it also satisfies the KKT conditions for USER(i), for all $i\in [N]$, and CLOUD problems with $m_{it}^k = z_{it}^k/\lambda, \q=\bmu, \p=\bl$ and $\bb=\mathbf\alpha$.
\vip{Prove the reverse!}
\end{proof}

\begin{algorithm}[ht]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\Input{Total number of machines $M$, step-size $\kappa$, error tolerance $\epsilon$, gradient steps $G$, job sizes $J_i$, CPT weighing $w_i(\cdot)$, and utilities $U_i(\cdot)$ (known only to user $i$ for $i\in[N]$)}
\textbf{Initialization}: Cloud service provider shows some initial prices $\q = \q_0\in\R^T$ (say, the all ones vector)\\
  \While{$\|\q - \q_{prev}\| \geq \epsilon\|\q_{prev}\|$}{
$\q_{prev} = \q$\\
Users, for all, $i\in [N]$, solve for budget vector $\m_i\in \R^T$ using the price vector $\q$ in the USER(i) problem\\
The cloud service provider receives the budget matrix $\m$ and does the following\\
step = 0\\
\While{step $\leq G$}
{$q_t = \max\left[q_t + \kappa\left(\frac{\sum_{k=1}^K\sum_{i=1}^N m_{it}^k\delta_k}{q_t} - M_t\right),0\right]~\forall~t\in [T]$\\
$step = step + 1$
}
}
% $\q^* = \q, \m^* = \m$\\
$z_{it}^k = m_{it}^k/q_t$ for all $i\in[N], t\in [T]$\\
Use Algorithm \ref{algo:proj_cpt} to project $z_{it}^k$ to the constraint sets $\sum_k\sum_i z_{it}^k \leq M_t, ~\forall~t$ and $z_{it}^k \geq 0~\forall~i,t,k$. \\
\KwResult{Solution to SYS, that is, the optimal pricing vector $\q^*$ and the optimal resource allocation vector $\x^*$}
 \caption{Finding the optimal resource allocation and pricing without utility information at the cloud end}
 \label{algo:price_tracking_cpt}
\end{algorithm}

\begin{algorithm}[ht]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\Input{$\z \in\R^{K\times N\times T}$, Constraint sets $C_1, C_2 \in \R^{K\times N\times T}$, where $C_1 := \{z_{it}^k |~\sum_k\sum_i z_{it}^k \leq M_t, ~\forall~t\}$, and $C_2 := \{z_{it}^k|~z_{it}^k \geq 0~\forall~i,t,k\}$, error tolerance $\epsilon$}
\textbf{Initialization}: Define $\z_1 = \z,~~~ \z_2 = \z$. \\
  \While{$\|\z - \z_{prev}\| \geq \epsilon\|\z_{prev}\|$}{
$\z_{prev} = \z$\\
$(\z_1')_{it}^k = z_{it}^k - \delta_k\max\left[\frac{\sum_{i,k}z_{it}^k\delta_k - M_t}{N\sum\delta_k^2}, 0\right]~\forall~i,t,k$.\\
$\z_2' = \z,~~~~ \z_2'[\z_2' < 0] = 0$ \\
$\z = (\z_1' + \z_2')/2$\\
$\z_1 = \z + \z_1 - \z_1'$\\
$\z_2 = \z + \z_2 - \z_2'$
}
\KwResult{$\z$: Projection of the input matrix to sets $C_1$ and $C_2$}
 \caption{Han's algorithm for projection on the intersection of convex sets}
 \label{algo:proj_cpt}
\end{algorithm}

\section{Experiments}


In this section, we present some experiments to show the advantages of considering a CPT based utility objective over a naive Expected Utility (EU) objective considered earlier. We consider the general CPT weighing function from Figure \ref{fig:2param_cpt} that is a function of two parameters, that is, for the $i$-th user, the CPT weighing is given by
$$w_{i}\left(p_{i}\right)=\frac{\delta p_{i}^{ \gamma_{i}}}{\delta p^{\gamma_{i}}+(1-p)^{\gamma_{i}}}.$$

For all the experiments in this section, we keep $\delta=0.7$ and $\gamma_i$ is chosen uniformly randomly in an i.i.d. fashion from $[0.3,0.5]$ for each user $i$. Further, we fix the number of users $N = 100$, the number of service tiers $T=5$, and the number of machines at the cloud provider $M_t = 1000,$ for all $t$. Each user obtains a utility between 50 and 100, uniformly chosen, upon successful completion of all her jobs.
In Fig. \ref{fig:2param_cpt_vs_eu_scale}, we plot the variation in utilities when the demand of the users is varied.  Initially, the number of jobs at the $i$-th user, $J_i$, is chosen to be a uniform random variable between 10 and 99 for all $i\in [1,100]$. However, to vary the demand, the number of jobs at each is multiplied by a scaling factor, and the overall utility of the system with the CPT objective (cite eqn) and EU objective (eqn) is plotted.

We see the when the jobs of users are scaled (i.e., the demand is increased while keeping the supply constant), the system utility with the CPT objective increases. In particular, when the demand and supply are almost the same, the CPT system utility is only $5.1\%$ better than the EU utility. However, when the demand of each user is scaled by a factor of five, the CPT system utility is $21\%$ better. For the rest of the experiments in this section, we consider the latter case (i.e., when the demand exceeds supply by a factor of five). 

In Fig. \ref{fig:2param_cpt_vs_eu}, we show the effect of having CPT users in the  system and how does that affect the overall system utility. Since the EU problem does the account for the CPT behaviour, the system utility does not change much. Further, we note that the cloud provider can significantly increase the system utility if it takes into account the CPT behaviour of the users.

\begin{figure}[t]
\begin{minipage}{.48\textwidth}
    \centering
    \includegraphics[scale=0.7]{figs_2param_n100_scale/system_utility_eu_vs_cpt_scale_PL_quant0_1.pdf}
    \caption{ CPT versus EU Utilities when the demand of the users is scaled.}
    \label{fig:2param_cpt_vs_eu_scale}
\end{minipage}
~
\begin{minipage}{.48\textwidth}
    \centering
    \includegraphics[scale=0.7]{figs_2param_n100_scale/system_utility_eu_vs_cpt_PL_quant0_1.pdf}
    \caption{ CPT versus EU Utilities when the percentage of users that exhibit CPT behavior is increased.}
    \label{fig:2param_cpt_vs_eu}
\end{minipage}
\end{figure}

\subsection{Market Simulations}

In this section, we run an experiment for 60 days with N = 100 users and T = 5 tiers, where each
day, users’ utilities are changing based on the market trends. Specifically, for the first 30 days,
we synthetically generate utilities that follow an upward trend based on the market following by
a downward trend for the next 30 days. To simulate this, we generate $u_{it}$, for all $i, t$, from a uniform
distribution in $[5, 10]$ in an i.i.d. fashion. The job size for the $i$-th user, $J_i$, for all $i$, is an i.i.d. integer chosen between 10 to 100 (which remains constant throughout the 60 days of the experiment) and $M_t = 5000$ for all $t$. To generate an upward market trend, we add 0.5 to $u_{it}, \forall i, t$, with probability
0.55 and -0.5 with probability 0.45 (the probabilities are flipped to generate a downward trend).

\begin{figure}[t]
        \centering
        \includegraphics[scale=0.8]{figs_2param_n100_scale/grad_vs_opt_vs_eu_vs_rand_util60_iter1.pdf}
        \caption{Sum utilities for the four resource allocation schemes}
\label{fig:market_sum_utility_2param_cpt}
\end{figure}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[scale=0.7]{figs_2param_n100_scale/grad_vs_opt_vs_eu_vs_rand_price_paid_user0_iter1.pdf}
        \caption{ Utility in the first tier across 60 days
        }
        \label{fig:2param_cpt_utils_tier0}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[scale=0.7]{figs_2param_n100_scale/grad_vs_opt_vs_rand_price_hour0_iter1.pdf}
        \caption{ Corresponding price charged by the cloud provider 
        }
        \label{fig:2param_prices_tier0}
    \end{subfigure}
    \caption{Utility and price charged in the first tier for the four resource allocation schemes}
\label{fig:market_tier0}
\end{figure*} 

We compare the following four schemes:
\begin{itemize}
    \item {\bf Optimal CPT pricing}: Here, we assume that the cloud provider is able to solve for the optimal lotteries and maximize system utility by utilizing the knowledge of users' utilities at each day. 
% Hence, the resource allocation is optimal which maximizes the sum utility of the system.
\item {\bf Price Tracking (CPT)}: In this case, the users' utilities are not known, and the cloud provider tracks users' utilities based on their budget signals (as described in Algorithm \ref{algo:price_tracking_cpt}). 
The cloud provider is assumed to update the prices everyday.
\emph{Users send budget signals only once per day.} These budget signals depend on the user's utility function on that day and the prices published by the cloud on that day.

\item {\bf Price Tracking (EU)}: Here, we do not consider the CPT-ness of users and use the price tracking algorithm from earlier work.

\item {\bf First-come-first-serve}: 
%This scheme is currently employed by many serverless service providers, such as AWS Lambda, Microsoft Azure Functions and Google cloud functions. 
Here, the pricing of the resources remains constant (as currently employed by most commercial service providers). 
%throughout the 60 days  
%(that is, it does not capture the mood of the market) 
% We take them to be 
It is the optimum prices determined by the utilities on day 1 and does not capture the mood of the market.
% for the purpose of simulations. 
Each day, the users are allocated resources on a first-come-first-serve (which is assumed to be random in order) or a lottery basis. 
\end{itemize}



==> hard_const_relax.tex <==
%!TEX root = main.tex

\section{Hard Constraint Problem Relaxation}
\label{sec: hard_const_relax}




With this interpretation in terms of $[K]$ alternatives, we get the following problem:
\begin{align}
\text{\bf\underline{SYS-CPT-K}} \nn \\
\max_{\substack{
\x^k \geq 0,\forall k,\\
\pi_i,\forall i,\\
T_i^k, \tilde T_i^k, \forall i,k 
}} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k U_i^{\tilde T_i^k} \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} x_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K],\\
 & \sum_{i=1}^{N} x_{it}^k \leq M_{t}, ~\forall ~t \in[T], k \in [K],\\
 & T_i^k := \min \{t \in [T] : \sum_{s = 1}^t x_{is}^k \geq J_i \}, ~\forall~i \in [N], k \in [K],\\
 & \tilde T_i^k = T_i^{\pi_i(k)},~\forall~i \in [N], k \in [K],\\
 & {\tilde T_i^1} \leq {\tilde T_i^2} \leq  \dots \leq {\tilde T_i^K}, ~\forall i \in [N].
\end{align}

We now use the relaxation trick as in the previous section.
We approximate the utility for user $i$ corresponding to alternative $k$ as follows:
\begin{align}
%\label{eq: cpt_approx}
    U_i^{T_i^k} \approx \sum_{t = 1}^T \frac{x_{it}^k U_i^t}{J_i}.
\end{align}
Note that when $(x_{it}^k, t \in [T])$ is $1$-sparse with that non-zero entry equal to $J_i$, the above approximation is exact.
With this relaxation our problem can be written as
\begin{align}
\text{\bf\underline{SYS-CPT-K-1}} \nn \\
\max _{\x^k \geq 0, \pi_i} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\x_{i}^{\pi_i(k)}) \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} x_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K],\\
 & \sum_{i=1}^{N} x_{it}^k \leq M_{t}, ~\forall ~t \in[T], k \in [K],
\end{align}
where $\bP(\x_{i}^k) = \sum_{t=1}^T x_{it}^k P_{it} = \sum_{t=1}^T x_{it}^k U_i^t/J_i$ and the permutation $\pi_i(k)$ is such that
$$ \bP_i(\x_i^{\pi_i(1)}) \geq \bP_i(\x_i^{\pi_i(2)}) \geq \cdots \geq \bP_i(\x_i^{\pi_i(K)}).$$
Note that the non-convex function $w_i(\cdot)$ is represented in the relaxed problem as constants $h_i^k$ due to discretization. However, the relaxed problem is still NP-hard since it requires an optimal permutation $\pi_i(k)$ to allocate the lotteries (we will discuss more on how to allocate lotteries with this formulation later). 

We now further relax the above problem by using the trick from \cite{phade2019optimal}.
This involves re-writing the problem by representing the permutations as a permutation matrix and relaxing them to doubly stochastic matrices.
We now give the details of this transformation.
%This gives rise to the following problem (see~\cite{phade2019optimal} for details of this transformation):
Corresponding to allocations $\x^k, \forall k \in [K]$ and permutations $\pi_i, \forall i \in [N]$, let $z_{it}^k := \x_{it}^{\pi_i(k)}$ be a $|T|$-dimensional column vector, for $i \in [N], k \in [K]$, and let $S_i$ be the $K \times K$ matrix given by $S_i(s,t) = 1$ if $\pi_i(t) = s$ and $S_i(s,t) = 0$ otherwise, for $s,t \in [K], i \in [N]$.
Note that $S_i$ is the permutation matrix corresponding to the permutation $\pi_i^{-1}$~(i.e. inverse of the permutation $\pi_i$).
Note that $S_i$ is also a doubly stochastic matrix.
Let $\Omega_K$ denote the set of all $K \times K$ doubly stochastic matrices, and
let $\Omega_K^*$ denote the set of all $K \times K$ permutation matrices.
Also note that the allocations $\x^k, \forall k \in [K]$ and the permutations $\pi_i, \forall \in [N]$ are uniquely defined by $\z := (z_{it}^k, i \in [N], t \in [T], k \in [K])$, and $S_i, i \in [N]$.
Let $\z_i^k := (z_{it}^k, t \in [T])$ and $\z_{it} := (z_{it}^k, k \in [K])$ denote column vectors.
Let $\1$ denote a column vector of dimension $K$.
The problem SYS-CPT-K-1 can equivalently be written as follows:
\begin{align}
\text{\bf\underline{SYS-CPT-K-2}} \nn \\
\max_{\z \geq 0, S_i \in \Omega_K^*} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\z_i^k) \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K],\\
 & \sum_{i=1}^{N} S_i \z_{it} \leq M_{t} \1, ~\forall ~t \in[T],\\
 &\bP_i(\z_i^1) \geq \bP_i(\z_i^2) \geq \cdots \geq \bP_i(\z_i^K).
\end{align}

We now relax the constraint $S_i \in \Omega_K^*$ to be $S_i \in \Omega_K$.
This gives us the following problem:
\begin{align}
\text{\bf\underline{SYS-CPT-K-3}} \nn \\
\max_{\z \geq 0, S_i \in \Omega_K} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\z_i^k) \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~ i \in[N],\\
 & \sum_{i=1}^{N} S_i \z_{it} \leq M_{t} \1, ~\forall ~t \in[T],\label{eq: sys_cpt_k_3}\\
 &\bP_i(\z_i^1) \geq \bP_i(\z_i^2) \geq \cdots \geq \bP_i(\z_i^K).
\end{align}

Notice that the constraint $\sum_{i=1}^{N} S_i \z_{it} \leq M_{t}$ implies that 
\[
    \frac{1}{K} \sum_{k=1}^K \sum_{i=1}^{N} z_{it}^k = \frac{1}{K} \sum_{i=1}^{N} \1^T S_i z_{it} \leq \1^T M_t \1 \leq M_t.
\]
If we replace constraint \eqref{eq: sys_cpt_k_3} by the above condition we get
\begin{align}
\text{\bf\underline{SYS-CPT-K-R}} \nn \\
\max _{\z^k \geq 0} ~~~~~& \sum_{i=1}^{N} \sum_{k=1}^{K} h_i^k \bP_i(\z_{i}^{k}) \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}^k \leq J_i, ~\forall~ i \in[N], k \in [K], \\
 &\frac{1}{K} \sum_{k=1}^K\sum_{i=1}^{N} z_{it}^k \leq M_{t}, ~\forall ~t \in[T],\\
 &\bP_i(\z_i^{k}) \geq \bP_i(\z_i^{k+1}), ~\forall~i \in [N], ~\forall ~1 \leq k \leq K-1. 
\end{align}



Notice that the problem SYS-CPT-K-R is an LP problem.
Besides, the value of the problem SYS-CPT-K-R is equal to the value of the problem SYS-CPT-K-2.
(Further details relating the primal and dual values the problems SYS-CPT-K-2, SYS-CPT-3 and SYS-CPT-R can be found in \cite{phade2019optimal}).

==> open_probs_old.tex <==
\section{Open Problems}
\subsection{Solving the problem SYS by finding the optimal ordering} 
Note that the optimal solution for the original problem SYS greedily allocates resources to the best user (not sure how best is defined yet). Thus, the task at hand is to find the optimal ordering of users to allocate resources to in a sequential fashion (i.e. until their jobs are complete). Corresponding to any permutation $\pi$ of the set $[N]$ we consider a greedy allocation scheme that dedicates maximum possible resources to the first agent in the permutation $\pi$ whose jobs have not been finished yet.
Formally, if $\{J'_i, i \in [N]\}$ are the jobs left for all players at time instant $t \geq 1$, i.e.
$J'_i = J_i - \sum_{s=1}^{t-1} x_{is},$
then
let 
$k_t := \min \{i \in [N] : \sum_{j = 1}^i J'_{\pi(j)} \geq M\},$
and
let $x_{\pi(j),t} := J'_{\pi(j)}$ for all $1 \leq j < k_t$ and let $x_{\pi(k_1), t} := M(t) - \sum_{j = 1}^{k_1 -1} J'_{\pi(j)}$.

Let $T_i^* :=  \min \{t \in [T] : \sum_{s = 1}^t x_{is}^* \geq J_i \}$ be the completion times corresponding to the optimal solution $x^*$ to SYS.
Let $\pi^*$ be a permutation of $[N]$ such that
\[
	T^*_{\pi^*(1)} \leq T^*_{\pi^*(1)} \leq \dots \leq T^*_{\pi^*(N)}.
\]
Since our cost function is such that the agents only care about their completion times, the greedy allocation corresponding to the permutation $\pi^*$ should have its value not more than $V^*$.
However, since $V^*$ is the minimum value, we get that the greedy allocation corresponding to $\pi^*$ has value $V^*$.
Thus we need to reframe our problem.

\vip{To be done: Given each agents parameters $J_i, v_i, \tilde T_i$, find the optimum permutation $\pi^*$ (not so easy).}

\subsection{Incentivizing Truthful Reporting}
Let $\pi(J_i, v_i, T_i)$ denote the optimum permutation corresponding to the agents parameters $J_i, v_i, \tilde T_i$.
Let us now consider special type of cost functions 
$$C_i(t) = v_i \1_{\{t > \tilde T_i\}} - v_i.$$ 
Equivalently we can think of
$$U_i(t) = v_i - v_i \1_{\{t \geq \tilde T_i\}} = v_i \1_{\{t \leq \tilde T_i\}},$$
as the utility function for agent $i$.
Here $v_i$ is the value the agent gets from having the job completed as long as it is completed before her threshold time $\tilde T_i$.
Since the agents will be reporting their parameters $J_i, v_i, \tilde T_i$ we would like them to be truthful.
We will say that truthful reporting is incentive compatible if each player benefits the most by reporting truthfully. 
As observed in the mechanism design literature, we need to introduce a payment mechanism to achieve this.
We will say that a payment mechanism is individually rational if each player is incentivised to participate in the mechanism.

\vip{Find a payment mechanism $P_i(J,v,\tilde T)$ that implements $\pi(J_i, v_i, T_i)$ and such that truthful reporting is incentive compatible for each player (and also individually rational).}

Here the the payment $P_i(J,v,\tilde T)$ is the amount agent $i$ plays for her jobs.
We have allowed it to be a function of the other players reports too, $J = \{J_1, \dots, J_N\}$, $v = \{v_1, v_2, \dots, v_N\}$, $\tilde T = \{\tilde T_1, \dots, \tilde T_N\}$.
Also the pricing is personalized, as in, it can be a different function for different players.
We should consider restrictions of the payment mechanism such that ones which are not personalized, or the ones in which $P_i(\cdot)$ depends only on agent $i$'s reports.

\vip{Find a payment mechanism $P_i(J,v,\tilde T)$ that maximizes the revenue $\sum_{i = 1}^N P_i(J,v,\tilde T)$ and such that truthful reporting is incentive compatible for each player (and also individually rational).}

\subsection{FLexible SLAs and their pricing}
Service level agreements can be viewed as lotteries over different types quality of service.
For example, a typical SLA would provide a customer certain probabilistic guarantees on his job completion and the corresponding charges.
There has been a growing evidence that people react in different ways to such uncertainties which further affects their decisions.
Cumulative prospect theory, a decision making model proposed by Tversky and Kahneman \cite{tversky1992advances} for which they won the Nobel prize, is particularly useful to accommodate customers' preferences and behavior.
Recent work on optimal resource allocation through lotteries \cite{phade2019optimal} is especially relevant in designing flexible SLAs along with an appropriate pricing scheme.


==> prob_from_old.tex <==
%!TEX root = ../main.tex

\section{Problem Formulation}

Suppose there are $N > 0$ agents $[N] := \{1, 2, \dots, N\}$ with their corresponding jobs of sizes $J_1, J_2, \dots, J_N$ respectively.
Let there be a server who can serve a maximum of $M$ jobs combined across different agents at each time instant $t \geq 1$.
Let $T := \lceil (\sum_{i = 1}^N J_i)/M \rceil$.
This is the maximum time needed if the server is never idle.
Let $x_{it}$ denote the number of jobs completed for agent $i \in [N]$ at time instant $t \in [T] := \{1, 2, \dots, T\}$.
Then $T_i := \min \{t \in [T] : \sum_{s = 1}^t x_{is} \geq J_i \}$ is the time it takes to complete agent $i$'s jobs.
Let $C_i(t)$ denote the cost incurred by agent $i$ if her jobs are completed at time instant $t$.
We will assume the function $C_i: [0, \infty) \to \bbR$ to be non-decreasing.
We will consider the problem of allocating resources $x_{it}$ to the agents in return of certain payments with the following two goals in mind:
\begin{enumerate}
	\item Minimize total cost incurred by all the agents.
	\item Maximize the revenue collected through payments.
\end{enumerate}

We can formulate a system problem for the first case as follows:
\begin{equation*}
\begin{aligned}
& \text{SYS}\\
& \text{Minimize}
& & \sum_{i=1}^n C_i(T_i)\\
& \text{subject to} && T_i := \min \{t \in [T] : \sum_{s = 1}^t x_{is} \geq J_i \}, \forall i \in [N],\\
&&& \sum_{i = 1}^N x_{it} \leq M, \forall t \in [T],\\
&&& x_{it} \geq 0, \forall i \in [N], t \in [T].
\end{aligned}
\end{equation*}

Let $c_{it} = C_i(t) - C_i(t-1)$ for all $i \in [N], t \in [T]$.
We can rephrase the system problem SYS as an integer linear programming problem as follows:
\begin{equation*}
\begin{aligned}
& \text{SYS-LP}\\
& \text{Minimize}
& & \sum_{i=1}^n c_{it}y_{it}\\
& \text{subject to} && y_{it} \geq 1 - \frac{\sum_{s = 1}^t x_{is}}{J_i}, \forall i \in [N], t \in [T],\\
&&& \sum_{i = 1}^N x_{it} \leq M, \forall t \in [T],\\
&&& x_{it} \geq 0, \forall i \in [N], t \in [T],\\
&&& y_{it} = 0 \text{ or } 1, \forall i \in [N], t \in [T].
\end{aligned}
\end{equation*}
Here, $y_{it}$ is an indicator that denotes if agent $i$'s are completed or not.
Let us relax the problem SYS-LP by replacing the constraint $y_{it} = 0 \text{ or } 1$ by $y_{it} \geq 0$.
\begin{equation*}
\begin{aligned}
& \text{SYS-LP-R}\\
& \text{Minimize}
& & \sum_{i=1}^n c_{it}y_{it}\\
& \text{subject to} && y_{it} \geq 1 - \frac{\sum_{s = 1}^t x_{is}}{J_i}, \forall i \in [N], t \in [T],\\
&&& \sum_{i = 1}^N x_{it} \leq M, \forall t \in [T],\\
&&& x_{it} \geq 0, \forall i \in [N], t \in [T],\\
&&& y_{it} \geq 0, \forall i \in [N], t \in [T].
\end{aligned}
\end{equation*}

Let $V^*$ be the optimum value for the problem SYS.
It is easy to see that the optimum value for the problem SYS-LP is also $V^*$.
Let $V^R$ denote the optimum value for the relaxed problem SYS-LP-R.
It is clear that $V^R \leq V^*$.
Let $x, y \in \bbR^{N \times T}$ be matrices with its entries given by $x_{it}, y_{it}$ respectively.
Let $x^R, y^R$ achieve the optimum value $V^R$ in SYS-LP-R.
We define $\hat y \in \bbR^{N \times T}$ with entries
\[
	\hat y_{it} := \begin{cases}
		0, \text{ if } y^R = 0,\\
		1, \text{ if } y^R > 0.
	\end{cases}
\]
We can check that $x^R, \hat y$ is a feasible solution for SYS-LP. Let $\hat V$ denote the value of SYS-LP at $x^R, \hat y$.
Then we have $V^R \leq V^* \leq \hat V$.
Note that $\hat V$ depends on the choice of $x^R, y^R$ that achieves the optimum in SYS-LP-R (there can be multiple $x,y$ that solve SYS-LP-R).\\

{\bf Question:} Can we bound the inequality gaps in $V^R \leq V^* \leq \hat V$?\\


Corresponding to any permutation $\pi$ of the set $[N]$ we consider a greedy allocation scheme 
that dedicates maximum possible resources to the first agent in the permuation $\pi$ whose jobs have not been finished yet.
Formally, if $\{J'_i, i \in [N]\}$ are the jobs left for all players at time instant $t \geq 1$, i.e.
$$J'_i = J_i - \sum_{s=1}^{t-1} x_{is},$$
then
let 
$$k_t := \min \{i \in [N] : \sum_{j = 1}^i J'_{\pi(j)} \geq M\},$$ 
and
let $x_{\pi(j),t} := J'_{\pi(j)}$ for all $1 \leq j < k_t$ and let $x_{\pi(k_1), t} := M - \sum_{j = 1}^{k_1 -1} J'_{\pi(j)}$.

Let $T_i^* :=  \min \{t \in [T] : \sum_{s = 1}^t x_{is}^* \geq J_i \}$ be the completion times corresponding to the optimal solution $x^*$ to SYS.
Let $\pi^*$ be a permutation of $[N]$ such that
\[
	T^*_{\pi^*(1)} \leq T^*_{\pi^*(1)} \leq \dots \leq T^*_{\pi^*(N)}.
\]
Since our cost function is such that the agents only care about their completion times, the greedy allocation corresponding to the permutation $\pi^*$ should have its value not more than $V^*$.
However, since $V^*$ is the minimum value, we get that the greedy allocation corresponding to $\pi^*$ has value $V^*$.
Thus we can reframe our problem:\\

{\bf Question:} Find the optimum permutation $\pi^*$.\\

Let us now consider special type of cost functions 
$$C_i(t) = v_i \1_{\{t > \tilde T_i\}} - v_i.$$ 
Equivalently we can think of
$$U_i(t) = v_i - v_i \1_{\{t \geq \tilde T_i\}} = v_i \1_{\{t \leq \tilde T_i\}},$$
as the utility function for agent $i$.
Here $v_i$ is the value the agent gets from having the job completed as long as it is completed before her threshold time $\tilde T_i$.\\

{\bf Question:} Given each agents parameters $J_i, v_i, \tilde T_i$, find the optimum permuation $\pi^*$.\\

Let $\pi(J_i, v_i, T_i)$ denote the optimum permutation corresponding to the agents parameters $J_i, v_i, \tilde T_i$.
Since the agents will be reporting their parameters $J_i, v_i, \tilde T_i$ we would like them to be truthful.
We will say that truthful reporting is incentive compatible if each player benefits the most by reporting truthfully. 
As observed in the mechanism design literature, we need to introduce a payment mechanism to achieve this.
We will say that a payment mechanism is individually rational if each player is incentivised to participate in the mechanism.
\\


{\bf Question:} Find a payment mechanism $P_i(J,v,\tilde T)$ that implements $\pi(J_i, v_i, T_i)$ and such that truthful reporting is incentive compatible for each player (and also individually rational).\\

Here the the payment $P_i(J,v,\tilde T)$ is the amount agent $i$ plays for her jobs.
We have allowed it to be a function of the other players reports too, $J = \{J_1, \dots, J_N\}$, $v = \{v_1, v_2, \dots, v_N\}$, $\tilde T = \{\tilde T_1, \dots, \tilde T_N\}$.
Also the pricing is personalized, as in, it can be a different function for different players.
We should consider restrictions of the payment mechanism such that ones which are not personalized, or the ones in which $P_i(\cdot)$ depends only on agent $i$'s reports.\\


{\bf Question:} Find a payment mechanism $P_i(J,v,\tilde T)$ that maximizes the revenue $\sum_{i = 1}^N P_i(J,v,\tilde T)$ and such that truthful reporting is incentive compatible for each player (and also individually rational).\\


==> proof_prop_typical_lottery.tex <==
%!TEX root = main.tex

\section{Structure of Typical Lottery Allocation}
\label{sec: proof_prop_typical_lottery}



We will decompose the problem SYS-CPT-K-R into user problems and a central problem in order to decouple the the different users.
Here we will use a different decomposition from the one that we used earlier.

\begin{align}
\text{\bf\underline{USER (i)}} \nn \\
\max_{\z_i^k \geq 0} ~~~~~&  \sum_{k=1}^{K} h_i(k) \bP_i(z_{i, \bullet}({k})) - \frac{1}{K} \sum_{k = 1}^K \sum_{t = 1}^T  \bar \rho_{it} z_{it}(k) \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{t=1}^{T} z_{it}(k) \leq J_i, ~\forall~  k \in [K], \label{eq: user_cpt_lp_r_1}\\
 %&\frac{1}{K} \sum_{k=1}^K z_{it}^k = \bar z_{it}, ~\forall ~t \in[T],\label{eq: user_cpt_lp_r_2}\\
 &\bP_i(z_{i, \bullet}({k})) \geq \bP_i(z_{i, \bullet}({k+1})), ~\forall ~1 \leq k \leq K-1 \label{eq: user_cpt_lp_r_3}.
\end{align}

\begin{align}
\text{\bf\underline{CENTRAL}} \nn \\
\max_{z_{it}^k \geq 0} ~~~~~& \sum_{i=1}^{N} \frac{1}{K} \sum_{k = 1}^K \sum_{t = 1}^T \bar \rho_{it} z_{it}^k \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& \sum_{i=1}^{N} \frac{1}{K} \sum_{k = 1}^K z_{it}^k \leq M_{t}, ~\forall ~t \in[T].\label{eq: net_cpt_lp_r_2}
\end{align}


We will first show that there exists equilibrium prices $\bar \rho_{it}$ such that any solution $\z$ to SYS-CPT-K-R is a common solution to USER(i), for all $i$, and CENTRAL problems, and vice versa, i.e. a common solution to to USER(i), for all $i$, and CENTRAL problems is a solution to SYS-CPT-K-R.
This essentially follows from showing that the complementary slackness conditions match.

This decomposition allows us to decouple the preferences of the different users. 
Note that the preference features of each player, namely, her utility and probability weighting functions, appear in her corresponding CPT-USER problem. And the CENTRAL problem correlates different players' preferences via psuedo prices $\bar \rho_{it}$.
We will use this decomposition to study the typical lottery-allocation received by a player by analysing the CPT-USER(i) problem.


For $Z_i \geq 0$, let us define
\begin{align}
V_i(Z_i) &:= \max_{\bar z_{it} \geq 0} ~~~~~ \sum_{t =1}^T P_{it} \bar z_{it}\nn \\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
&\text{subject to} ~~~~~  \sum_{t = 1}^T  \bar \rho_{it} \bar z_{it} \leq Z_i, \nn\\
&~~~~~~~~~~~~~~~~~~~~~\sum_{t=1}^{T} \bar z_{it} \leq J_i. \nn
\end{align}

The USER(i) problem can now we written as
\begin{align}
\text{\bf\underline{USER (i)}} \nn \\
\max_{\z_i^k \geq 0} ~~~~~&  \sum_{k=1}^{K} h_i(k) V_i(Z_i(k)) - \frac{1}{K} \sum_{k = 1}^K Z_i(k) \nn\\
% \maxi_{x_{it}\geq 0}  \sum_{i=1}^n U_i^{T_i}\nn \\
\text{subject to} ~~~~~& V_i(Z_i({k})) \geq V_i(Z_i({k+1})), ~\forall ~1 \leq k \leq K \label{eq: user_cpt_lp_r_3},
\end{align}
where $Z_i({K+1})$ is the zero vector of $T$-dimension.


We now observe that the function $V_i(\cdot)$ is non-decreasing and concave. Include a proof here.
Now similar to the proof in \cite{phade2019optimal}, we can show that 
\[
	V_i(Z_i({k^*})) = V_i(Z_i({k^* + 1})) = \dots = V_i(Z_i({K})).
\]
This proves proposition~\ref{prop: typical_lottery}.

